Automated Deobfuscation of Android Native Binary Code

With the popularity of Android apps, different techniques have been proposed to enhance app protection. As an effective approach to prevent reverse engineering, obfuscation can be used to serve both benign and malicious purposes. In recent years, more and more sensitive logic or data have been implemented as obfuscated native code because of the limitations of Java bytecode. As a result, native code obfuscation becomes a great obstacle for security analysis to understand the complicated logic. In this paper, we propose DiANa, an automated system to facilitate the deobfuscation of native binary code in Android apps. Specifically, given a binary obfuscated by Obfuscator-LLVM (the most popular native code obfuscator), DiANa is capable of recovering the original Control Flow Graph. To the best of our knowledge, DiANa is the first system that aims to tackle the problem of Android native binary deobfuscation. We have applied DiANa in different scenarios, and the experimental results demonstrate the effectiveness of DiANa based on generic similarity comparison metrics.

==> Automated Deobfuscation of Android Native Binary Code/Section1-Intro.tex <==
\section{Introduction}

% Para1: Android apps grow explosively, could be developed in both Java and C++
% Android applications (apps) have seen wide spread adoption recent years. The number of apps in Google Play has surpassed 3.5 Million mark by the end of April 2018~\cite{AppNumber}. Android PacKage (APK) is the package file format used by the Android Operating System for distribution and installation of mobile apps. APKs are generally written in Java, while Android also supports incorporating native code binaries (written in C/C++) as part of the apps to boost app developing process. 

%% native code
Android apps have received widespread adoption recently \cite{AppNumber}. Besides the standard Android programming model in Java, Android NDK \cite{NDK} was introduced to allow developers to include native code binaries (write in C/C++) in their apps.


% Android apps are easy to be cracked and modified, as many reverse engineering tools available in the community~\cite{apktool, androguard, dex2jar}. A large mount of previous work~\cite{jiang2012dissecting, wang2015wukong} suggested that app repackaging is a major way for malware spreading. To increase the effort of reverse engineering and hinder cracking, and prevent theft of intellectual property, code obfuscation techniques are widely used in Android apps [CITE HERE]. Many tools exist that allow developers to obfuscate their apps [CITE Proguard
% DashO Dexguard DexProtector ApkProtect Shield4j Stringer Allitori]. For example, ProGuard is the most popular obfuscation tool that integrated into the Android build system. These obfuscators operate at different levels, e.g., Java source code level, Java bytecode level, Dex bytecode level and native code level.

% Although many legitimate apps use code obfuscation techniques to prevent their apps being cracked, Android malware also take advantage of these techniques to evade detection and to hinder reverse engineering by security analysts. It is reported that malicious Android apps that use heavy obfuscation techniques found in Google Play from time to time [CITE HERE].

% Thus, several fellow researchers in our community focused on the deobfuscation of Android apps. For example, DeGuard was proposed to reverse layout obfuscation (naming obfuscation) [CITE HERE] that generated by ProGuard. Their key idea is to learn a probabilistic model over a large mount of non-obfuscated apps and to use this probabilistic model to deobfuscate new APKs. Layout obfuscation is the easiest method in Android app obfuscation, which does not alter the program logic (e.g., control flow and data flow) of the apps. To the best of our knowledge, all of the existing studies focus on the Java code level deobfuscation. 

Recent work suggested that native code had been widely used~\cite{sun2014nativeguard, alam2016droidnative, afonso2016going} in Android apps, which severely complicates the process of static analysis. As Java bytecode can be easily decompiled, malware developers usually hide the malicious payload and core functionalities in the native code to evade detection~\cite{malware1, malware2, malware3, afonso2016going}. 
Even worse, native code can also be obfuscated, which further increases the difficulty of security analysis. For example, the towelroot exploit (CVE-2014-3153)~\cite{Towelroot1, CVE2014}, one of the biggest Root Exploits family in Android, was found obfuscated at the native code level by O-LLVM. It took a lot of efforts for security researchers to dive into the technical details of the code due to obfuscation. Figure~\ref{fig:motivating} shows the control flow graph of an obfuscated function ``search\_goodnum'', which is one of the key components of a Proof-of-Concept (PoC) implementation of the towelroot exploit. Apparently, the obfuscated control flow becomes too complex to understand the real logic. 

Although several attempts~\cite{Bichsel2016Statistical, Baumann2017Anti} have discussed the deobfuscation of Android apps, all of them have been focused on Java-level deobfuscation.
% (either Java source code or bytecode). 
For example, DeGuard~\cite{Bichsel2016Statistical} was proposed to reverse layout obfuscation (naming obfuscation) generated by ProGuard. Their key idea is to learn a probabilistic model over a large number of non-obfuscated apps and to use this model to deobfuscate new APKs. Layout obfuscation is the easiest one in Android app obfuscation, which does not alter the program logic (e.g., control flow) of the apps. To the best of our knowledge, no previous studies have attempted to tackle native code deobfuscation for Android yet. 
% \YG{How about other work besides DeGuard??}



\begin{figure}[t]
\centerline{\includegraphics[width=0.48\textwidth]{pictures/motivation.png}}
%%\vspace{-0.1in}
\caption{The CFG of an obfuscation function in POC of the TowelRoot exploit.}
%\vspace{-0.2in}
\label{fig:motivating}
\end{figure}

\textbf{Motivation.} The focus of this paper is deobfuscating the native code in Android apps. To be specific, we focus on the deobfuscation of native code that was protected by Obfuscator-LLVM (O-LLVM), which is the most popular native code obfuscator. O-LLVM is a set of obfuscating code transformations suite, which is implemented as middle-end passes in the LLVM compilation flow. O-LLVM offers three obfuscating methods: Instruction Substitution (InsSub), Bogus Control Flow (BCF) and Control Flow Flattening (CFF). Many popular packing tools, e.g., Baidu Jiagu~\cite{baidujiagu} and Bancle~\cite{Bangcle}, are implemented based on O-LLVM. 
% \haoyu{One or two sentences here to briefly describe OLLVM.---done} 
% \haoyu{Briefly describe two related work here.}

\textbf{Challenges.} Binary code deobfuscation is not a new task introduced in Android, as many studies have already been proposed for PC platforms (e.g., x86). Udupa \textit{et al.}~\cite{udupa2005deobfuscation} use static techniques to remove the dead edges added by the obfuscator. Yadegari \textit{et al.}~\cite{yadegari2015generic} proposed a deobfuscating approach based on the execution trace of the executable code. 
However, it is non-trivial to deobfuscate Android native binary code because there are no existing deobfuscation tools that can deal with full O-LLVM obfuscation, especially in the scenario of Android apps and for the ARM platform. Specifically, we face the following main challenges in this work:
\begin{itemize}
\item 
\textbf{Complexity due to instruction optimization on ARM}. Due to the specific optimizations on the ARM platform, some obfuscated operations may not be independent. It may be interleaved with normal instructions and operations. 
Thus it becomes a challenge to comprehensively and accurately pinpoint the obfuscated instructions. 
% 由于arm平台的优化，导致混淆的部分与原始信息的混合复用，如何在这种情况下将两者区别开来，并恢复混淆部分，成为了我们首先面对的问题。

% \haoyu{rewrite}
\item 
\textbf{Difficulty in control flow recovery due to basic block splitting}.
%  and basic block splitting 
% 由于ollvm的混淆使用分发器对原始基本块进行调度，在这种情况下上下文的继承关系就显得特别重要，如何在尽可能多的继承上下文信息，并不造成路径爆炸，也成为了一个关键的challenge
Control Flow Flattening in O-LLVM obfuscation can completely destroy the original control flow. At the same time, original basic blocks can also be split or partially merged, which may cause the separation of original semantic information. It becomes difficult to properly recover control flow in this kind of situations.
% OLLVM可以将原始控制流摧毁，并且原始的基本块在混淆程序中会被拆分和部分复用，从而造成携带信息与原始信息的差异。如何在这种情况下正确的恢复控制流。
% 由于OLLVM的反混淆工作是flow-sensitive的，在符号执行时，由于路径约束的不确定性，直接的符号执行会造成路径爆炸的问题，如何尽可能多的保留上下文信息，并不造成路径的爆炸，也成为了一个关键的challenge
\item 
% \textbf{How to perform flow-sensitive symbolic execution}.\haoyu{rewrite}
\textbf{Challenges in symbolic execution due to unknown path constrains}.
We will apply symbolic execution as one of the key steps in deobfuscation for the purpose of systematically exploring multiple program paths, similar as in previous work~\cite{guillot2010automatic,xu2017cryptographic,gabriel2014deobfuscation}. However, since the recovering process of O-LLVM obfuscated binary is flow-sensitive, incomplete context information may lead to incomplete or wrong path exploration,
while performing symbolic execution directly will cause the path explosion problem. Thus we need to find a way to retain the context information as much as possible, while avoiding path explosion during symbolic execution.

% How to maximize the context inheritance during the process of recovering the original control flow becomes a key challenge of our work.
% \footnote{For example, the constraint and calculation in a basic block may be separated into two blocks. It can only obtain incomplete information when analyze a }

% Thus, the context inheritance become particularly important in the recover process. How to inherit the context information as much as possible and do not cause the path explosion also became a key challenge.
% \haoyu{A short title here to name the challenge.}

% \item \textbf{Hybrid Obfuscation Techniques.} In general, malware developers could take advantage of hybrid obfuscation techniques to generate a robust malware sample. As O-LLVM provided different techniques to obfuscate code in both instructions and control flow aspect, how to identify what obfuscation techniques are used, and perform the deobfuscation actions at hybrid cases (rather than obfuscation-specific approach), has remained as a challenge.
% (\haoyu{briefly describe what is pass here}) 
% 对于ollvm多种情况混合的时候，如何进行特征判定，进而进行后续的恢复工作也成为了我们工作中遇到的问题
% For the unknown of the analysis object in reality situation, how to judge the obfuscation approach of OLLVM, and then carry out the subsequent recovery work, has become a challenge in our work too.
\end{itemize}

\textbf{Approach}
In this paper, we propose DiANa (\underline{\textbf{D}}eobfusca-t\underline{\textbf{i}}on of \underline{\textbf{A}}ndroid \underline{\textbf{Na}}tive Binary Code), a new approach for automated deobfuscation of Android native binary code. 
% It uses the method of taint analysis and symbolic execution to recover the O-LLVM obfuscated Android native functions.
Technically, \Name works by combining static taint analysis and symbolic execution to remove the obfuscation introduced by different obfuscating techniques in O-LLVM. One key feature of \Name is that we introduce \textit{taint analysis} to perform semantic level deobfuscation, while considering both general and compiler optimization situation. We also exploit flow-sensitive \textit{symbolic execution} to rebuild the seriously obfuscated control flow. 
To overcome the challenge of basic block splitting, we chop the original control flow, select analysis targets through static features, and dynamically adjust the analysis target sequence to maximize context inheritance. 



% \YG{More on evaluation results HERE.}
% 为了克服基本块拆分带来的挑战，我们将原始控制流拆分，通过静态特征选择分析目标，并动态调整分析目标序列，以最大程度的继承上下文

% \haoyu{describe more about our system and how you overcome the challenges.}
% It is noticeable that DiANA also can detect what kinds of obfuscating approach are used and makes deobfuscation based on the 
% \haoyu{INTRODUCE SOME KEY TECHNIQUES HERE. How to solve the aforementioned challenges?}
% \begin{itemize}
% \item Approach1
% % 对ARM平台的混淆特征进行了全面的总结，包括多种pass进行混淆的情况
% \item Approach2
% % 对于OLLVM的部分混淆使用污点分析，将疑似混淆操作的寄存器置为taint，以应对arm的指令优化，确保反混淆的完整性
% \item Approach3
% % 对符号执行进行CFF反混淆的时候，对基本块序列的执行序列进行动态调整，以最大程度上的继承上下文
% \end{itemize}

Experiments on multiple benchmarks and real-world cases suggest that our approach can accurately deobfuscate native code obfuscated by O-LLVM. We believe \Name can be used by security analysts to make it easier to inspect native code, even if it was heavily obfuscated.
% In addition, evaluation proves that \Name works well with the hybrid obfuscation due to the comprehensive feature summary.
This paper makes the following major contributions:
\begin{itemize}
\item To the best of our knowledge, this is the first work to tackle native code deobfuscation in Android apps. Our approach is able to handle different obfuscations provided by O-LLVM, the most popular obfuscator for Android. 

\item We design and implement DiANa, a system that can successfully deobfuscate native code in Android apps. \Name leverages taint analysis to overcome the complication due to ARM-specific optimizations. It also deploys flow-sensitive symbolic execution to tackle  Control Flow Flattening obfuscation in O-LLVM. 
%   We have a set of optimization methods to both the deobfuscating process and the final output. These can not only improve the efficiency of deobfuscation work, but also make it easier to understand recovered results.
% We believe our research could help boost the native-level malware detection and analysis.
% \haoyu{need a contribution here}\textbf{\haoyu{suggest write the optimization/novel aspects of our work here}} 

\item Our evaluation on a set of Android apps demonstrates that \Name is effective in native code deobfuscation and could become a valuable tool for tasks including program analysis and malware detection.  
%We have implemented a deobfuscation system DiANa, and applied it to various benchmarks and real-world exploits to evaluate the effectiveness of our system. 
We will release our system and the benchmarks to the research community at: 
\url{https://github.com/DiANa-deobfuscation-2020/DiANa}
%%\footnote{The code of symbol execution in CFF is inspried by the deflat script of the GitHub user liumengdeqq on x86 platform.}
\end{itemize}

==> Automated Deobfuscation of Android Native Binary Code/Section2-BackgroundAndRelated.tex <==
\section{Background and Related Work}
\label{sec:background}

To the best of our knowledge, this is the first work that tackles Android native code deobfuscation in our community. Nevertheless, there are already many studies on code obfuscation and deobfuscation for applications on both mobile and PC platforms. 


\subsection{Android App Obfuscation}

To increase the bar for reverse engineering and hinder cracking, and prevent theft of intellectual property, code obfuscation techniques have been widely used in Android apps~\cite{dong2018understanding}, for both legitimate apps and malware.
Many tools allow developers to obfuscate their apps~\cite{proguard, DashO, DexGuard, DexProtector, allatori, junod2015obfuscator}. For example, ProGuard is a popular obfuscation tool integrated in the Android build system. These tools may operate at different levels, e.g., Java code level, Dex bytecode level and native code level.

Native code level protection is much stronger than Java-level protection, thus state-of-the-art commercial packers utilize native code obfuscation to increase the complexity of reverse engineering~\cite{duan2018things}. As a side effect, Android malware also take advantage of native code obfuscation to evade detection.

\textbf{Obfuscator-LLVM (O-LLVM)} is one of the most widely used code obfuscator for both x86 and ARM platforms~\cite{junod2015obfuscator}.
It is implemented as middle-end passes in the LLVM compilation process, which offers guaranteed compatibility with LLVM. 
% It was first introduced by Junod, P., et al.\cite{junod2015obfuscator} and open-sourced on Git-Hub\cite{githubollvm}. 
% \haoyu{should describe clear what is pass here.} 
It offers the following three obfuscation techniques: 
% \emph{Instruction Substitution}, \emph{Bogus Control Flow} and \emph{Control Flow Flattening}. 

\emph{\textbf{(1) Instruction Substitution (InsSub)}}.
InsSub is the simplest obfuscation technique in O-LLVM. It replaces the standard binary operations, e.g., arithmetic (ADD, SUB) or boolean ones (AND, OR and XOR), by functionally equivalent but more complicated sequences of instructions. 
For each kind of operations, there are multiple ways to perform obfuscation. InsSub chooses one at random to increase code diversification in the resulting obfuscated code. 

\emph{\textbf{(2) Bogus Control Flow (BCF)}.}
BCF modifies the CFG by adding a conditional jump to randomly selected basic blocks, which either points to the original basic block or to a fake basic block looping back to the conditional jump block\cite{junod2015obfuscator}. In order to evade detection and optimization by the optimizers, an opaque predicate~\cite{wiki:opaque} (i.e., a mathematical expression which always evaluating to the same value) is used to ensure that only the original basic block is executed during run-time. 

\emph{\textbf{(3) Control Flow Flattening (CFF)}.}
This is the most effective, and the most difficult to deobfuscate, pass in O-LLVM. The basic idea is to remove all easily identifiable conditional jumps (e.g., \texttt{IF-ELSE}) and looping structures (e.g., \texttt{WHILE,FOR}), and use a big switch construct to route the code control flow through the proper basic blocks. The flow dispatcher chooses the next block using a routing variable, which resets in each basic block and leads the flow to the next correct basic block. Besides, there is a compilation flag that enables further breaking the code structure by artificially increasing the number of basic blocks in a function.

In general, InsSub and BCF are both semantic obfuscations that work at the instruction level, while CFF is an overall remodeling of the control flow in a function.


\vspace{-0.1in}
\subsection{Mobile App Deobfuscation}

Although several attempts have been focused on the deobfuscation of Android apps, all of them deal with Java-level deobfuscation. DeGuard \cite{Bichsel2016Statistical} was proposed to deal with layout obfuscation introduced by ProGuard~\cite{proguard}. The key idea is to summarize a probabilistic model by learning unobfuscated apps on a large scale and then use the model to recover the obfuscated code. Also, Baumann \textit{et al.}~\cite{Baumann2017Anti} use a similar approach to perform ProGuard deobfuscation by code matching. However, layout obfuscation is the easiest, as it does not alter the program logic. 

\subsection{General Code Deobfuscation}

Binary code deobfuscation has been widely studied for the PC platforms (x86)~\cite{guillot2010automatic,likarish2009obfuscated,madou2006loco,yadegari2016automatic,kotov2018towards,david2017formal,gabriel2014deobfuscation,D-OLLVM2017,udupa2005deobfuscation,yadegari2015generic}.
The closest work related to ours might be the one proposed by Gabriel~\cite{gabriel2014deobfuscation}, which attempted to recover O-LLVM obfuscated code on the x86 platform. The work is based on the Miasm~\cite{miasm} framework to reverse the obfuscated function to a control flow graph. Similarly, some work ~\cite{D-OLLVM2017} ~\cite{decompiler_2017}
used similar idea based on different kind disassembler ~\cite{binaryninja, jeb}.
However, they did not tackle the challenges introduced by basic block splitting and instruction optimization, which pose a great challenge for both x86 and ARM platforms. Besides, they did not provide an effective method to identify the obfuscation techniques used in a binary. Finally, context inheritance and sub-function calls are not considered in their work, which is more likely to fail when analyzing large programs. Yadegari \textit{et al.}~\cite{yadegari2015generic} proposed a generic approach to automatically deobfuscate binary code on x86. They use the execution trace extracted from a specific dynamic analysis environment as the input of their system. As a result, their work is not suitable on analyzing shared libraries in Android projects because most shared libraries lack of main functions or entry points~\cite{wiki:Library}.


% Udupa \textit{et al.}~\cite{udupa2005deobfuscation} proposed to use static analysis for deobfuscating programs obfuscated by CFF on the x86 platform. Their work was based on an older version of CFF, which is different algorithm from the state-of-the-art technique\cite{o-llvm-git}\haoyu{cite}. Besides, they could only identify edges that was added by CFF, while CFF is a rebuild of the entire CFG, thus this approach does not seem to work now.
% Coogan \textit{et al.}~\cite{coogan2011deobfuscation} uses equational reasoning on assembly-level instruction semantics to simplify the obfuscation code from execution traces of emulation-obfuscated programs. 
% But it is difficult for their approach to extract the logic of the underlying operation into higher-level structures such as control flow graphs.



% . He studied the O-LLVM deobfuscating work on the x86 platform which has a good inspiration for our work. In his work, he proposed a basic study of deobfuscation on three passes of O-LLVM and used a simple example to illustrate the O-LLVM obfuscation effect on x86. He used the framework Miasm to reverse the obfuscated function to a control flow graph. 
% But obviously there are some shortcomings in his work. The first is that the platform is different. There are basic block splitting and instruction optimization on the ARM platform, which makes deobfuscating work difficult. Second, for the obfuscation involves InsSub and BCF, his work results only recovered into the graph. But our result can be written into binary, which is more advantageous for reverse analysis to obtain source code. And the decision features he used in CFF obfuscation are too singular, neither applicable to the ARM platform nor accurate on x86. Finally, in the symbolic execution part, there is a lack of context inheritance and sub-function call considerations, which makes it a drawback when analyzing large programs.

% 首先在反混淆工作上是有一些工作的，其中很多集中在x86平台上，例如




% While the standard programming model for Android apps is to write the apps in Java and distribute the bytecode, the Android NDK~\cite{NDK} is introduced to allows developers to include native code binaries (write in C/C++) as part of the apps. Android system provides an interface (JNI)~\cite{jni} for Java code to call functions of native code and vice versa. Native code could boost the app developing process, by reusing a large mount of legacy libraries that written in C/C++, or implementing CPU-intensive tasks (e.g., game graphic engines and signal processing) and interacting more directly with the kernel and hardware to improve overall performance of the app.


% The existence of native code severely complicates the static analysis of Android apps. Most of previous work only focused on app bytecode, thus malware developers can include the malicious payload in a native code component to evade detection [CITE HERE]. Besides, native code could be obfuscated by advanced obfuscation techniques, which greatly increase the effort for security analysis. To the best of our knowledge, no previous work has tackled the native code deobfuscation for Android apps before.

% \haoyu{will rewrite this part.}

% Native code level protection is much stronger than Java-level protection (e.g., ProGuard), \haoyu{TODO}
% thus all the commercial packers utilize native code obfuscation to increase the complexity of reverse engineering [CITE NDSS 2018]. 

% Recent reports found that many commercial packers (e.g., Baidu Packer [CITE HERE], one of the most popular packers in China) implement native code level protection based on O-LLVM. O-LLVM is a set of obfuscating code transformations suite. It implemented as middle-end passes\footnote{Passes perform the transformations and optimizations that make up the compiler in LLVM} in the LLVM compilation, which has guaranteed compatibility. It was first introduced by Junod, P., et al.\cite{junod2015obfuscator} and open-sourced on Git-Hub\cite{githubollvm}. 
% % \haoyu{should describe clear what is pass here.} 
% O-LLVM offers three obfuscating methods: Instruction Substitution, Bogus Control Flow and control Flow Flattening. 
% % \haoyu{methods, pass}

% \haoyu{Brief introduce OLLVM here. e.g., widely used, source code level. open source. platforms. how to use it in Android. etc...}

% \haoyu{It's better to show several small examples here.}


% As a result, the instruction substitution pass is suggested to run after all LLVM optimization passes. Also, substitution of floating-point operators is not supported because it brings additional numerical inaccuracy.
% \begin{table}[]
% \begin{tabular}{llll}
% \begin{tabular}[c]{@{}l@{}}a = b - (-c) \\ a = -(-b + (-c)) \\ a = b + r; a += c; a -= r\\ a = b - r; a += c; a += r\end{tabular} & a = b + c &  &  \\
% \begin{tabular}[c]{@{}l@{}}a = b + (-c)\\ a = -((-b) + c)\\ a = b + r; a -= c; a -= r \\ a = b - r; a -= c; a += r\end{tabular} & a = b - c &  &  \\
% a = (b ˆ ! c) \& b & a = b \& c &  &  \\
% a = (b \& c) | (b ˆ c) & a = b | c &  &  \\
% a = (!b \& c) | (b \&! c) & a = b ˆ a &  & 
% \end{tabular}
% \end{table}





% \subsection{Empirical Study of Native Code Obfuscation}


% Previous work [] suggested that native code is widely adopted by popular apps, and 86\% of the most popular Android apps contain native code. Nevertheless, we also want to make a large-scale empirical study to explore: \emph{(1) how many apps in the markets use native code and how many of them are OLLVM-obfuscated?} and \emph{(2) what is the difference between benign apps and malware on using native code?}


% \subsection{Related Work}



% Our work is mainly related to three lines of research: \emph{mobile app obfuscation}, \emph{mobile app deobfuscation} and \emph{general code deobfuscation}.



% \subsection{Mobile App Obfuscation}
% Due to the easy-to-reverse nature of Java, code protection for Android apps is of particular importance. As a result, most obfuscation work on Android is focus on Java code. There are four popular obfuscation approaches~\cite{dong2018understanding}: identifier renaming, string encryption, Java reflection, and packing. 


% \subsection{Mobile App Deobfuscation}
% % 说android上的反混淆方法，java层的
% 很多都是针对proguard的
% Statistical Deobfuscation of Android Applications，
% % 给出了一种针对java层的反混淆工具degurad，他们的侧重点在Layout Deobfuscation. 通过他们的工作，将在布局混淆中携带关键语义信息的被替换为没有语义含义的信息恢复


% \subsection{General Code Deobfuscation}

% 他们完成了一个很好的反混淆原型设计并在部分数据集上进行了验证，但他们的侧重点是针对虚拟化混淆的恢复。



% NOTE: Summarize related work based on the above categorization

% ========================
% 最后我们来说说


% 但明显他们的工作存在着一些弊端
% 1、首先是平台不一样，ARM平台上由于存在着基本块的拆分和指令的优化，
% 1、对于Ins和BCF，他们的工作只能恢复到CFG层级，而我们的可以写进binary。因为他们的工作基于的是Miasm的中间表达优化，而中间语言重写进binary是很难得





% android上没有什么针对native的反混淆工作，最后说与我们的工作最接近的是ollvm的反混淆研究，他是我们工作的启蒙。但由于arm平台本身的特点，例如基本快的拆分和指令的优化，以及ollvm版本的迭代，已经产生了一些变化。另外该工作对于符号执行的上下文继承也没进行关注。我们在此基础上XXXXXX

==> Automated Deobfuscation of Android Native Binary Code/Section3-SystemOverview.tex <==
\section{Approach Overview}
% \section{Native Code Deobfuscation}
% 我们对于ollvm的每一个pass都做了对应的恢复手段，值得注意的是，由于指令替换这个pass是最为简单的混淆手段，在我们的恢复手段中并不会针对他的loop>1的情况进行讨论，instead, our approach only focus on the official suggested setting.

% 这一节我们会介绍我们的方法的具体实现，首先将对反混淆系统的整体框架进行介绍，然后针对ollvm的每个pass，逐一介绍针对该pass的反混淆，各个系统是如何配合的
% In this section, we will elaborate our deobfuscation approach in specific details. Firstly, we will illustrate the overall framework of our O-LLVM deobfuscating system. 

% Second, because instruction substitution and bogus control flow are both semantic levels of instruction obfuscation, while control flow flatten is an overall change to the function control flow. In order to explain our method in detail and make it easy to understand, we will introduce how system works to deobfuscate each pass of O-LLVM separately.

% After that, due to the integrity of our deobufuscation system and the unknownness of actual input, we will illustrate the specific process of the actual situation analysis. 

% \haoyu{TODO: may need rewrite this part.}

% \subsection{System Architecture}

\textbf{Goal.}  We use the term \textbf{deobfuscation} to refer to the process of removing the effects of obfuscation from the native binary, and ideally recover the original code and control flow before obfuscation. For a given APK input, DiANa first extracts the native binary and determines whether it is obfuscated, then analyzes and transforms the code to obtain a functionally equivalent form that is simpler and easier to understand. For non-trivial code, the deobfuscation results is rarely the same as the original code, however, it is close to the original and much easier to understand compared to the obfuscated version.
% we use taint analysis to address the challenge that introduced by instruction optimization. 

\textbf{Key Techniques.}
To address the aforementioned challenges, we rely on taint analysis and enhanced symbolic execution to recover O-LLVM obfuscated code. 
Taint analysis is used to address the challenge introduced by instruction optimization, which performs global feature matching to comprehensively detect all obfuscations introduced by O-LLVM and identify instructions needed to be rewritten by tracking tainted registers.
Symbolic execution is used to reconstruct the control flow ruined by CFF. We first identify basic blocks that maintain original operations based on an ARM-specific basic block classification approach. Then we perform chopped symbolic execution \cite{trabish2018chopped} to address the path explosion challenge. Finally, we use dynamic queue scheduling to maximize the context inheritance and rebuild the original control flow by conducting flow-sensitive symbolic execution.
% 1\ chopped,2\arm based
% To solve the challenge that introduced by basic block splitting, an ARM-based classification approach is proposed. Due to the recover process is flow-sensitive, we use a dynamic exchanging model to make recovery more accurate. 




\begin{figure}[t]
\centerline{\includegraphics[width=0.3\textwidth]{approach_pic/system-new-v3.png}}
%%\vspace{-0.1in}
\caption{Overall architecture of DiANa.}
%%\vspace{-0.2in}
\label{system}
\end{figure}





\textbf{Overall Architecture.}
Fig. \ref{system} illustrates the system architecture of \Name that is mainly composed of four parts. During the pre-processing stage, \Name first determines what kinds of obfuscation techniques are used in the input binary. Then it performs semantic level deobfuscation for InsSub and BCF based on mainly taint analysis. For the binaries protected by CFF, \Name will perform chopped flow-sensitive symbolic execution to rebuild the control flow. Then the recovered control flow will be optimized in consideration of basic block splitting. All the deobfuscation results will be integrated and rewritten to the binary(or control flow graph) in the end.

% Then extract necessary features that need to be used in the following  


% Feature Extractor, Taint Analyzer, Flow Analyzer and Re-builder.

% As shown in Figure.\ref{system}, \Name is mainly composed of four subsystems: Feature Extractor, Taint Analyzer, Flow Analyzer and Re-builder.

% \textbf{\textit{Feature Extractor}} is the preprocessor of our deobfuscating system. For the input raw function, it will first extract static features, including opcodes, operands and control flow, to determine whether the input is O-LLVM obfuscated or not, and what obfuscating techniques in O-LLVM are used. 
% After that, all needed information will be saved and passed to the next subsystem.

% This part extracting semantical features from the original binary. Such as the 
% 对于输入的原始函数，Semantical Feature Extractor会先对其进行特征提取，包括指令和操作数层面和CF层面的，以判断该输入是否为ollvm混淆，并确定混淆手段是什么。之后，Semantical Feature Extractor会将这些后续工作所需要的信息传入Flow Analyzer

% This part mainly works to deobfuscate instruction substitution。我们针对ollvm的指令替换的5种模式，设计了

% \textbf{\textit{Taint Analyzer}} is mainly used to remove the obfuscation of instruction substitution and bogus control flow. It is responsible for discovering the general forms and variants of these two ways of obfuscation. It will also set registers involved in the obfuscating operation in the analysis process as tainted to determine the patching position, which ensures the original context not being corrupted. 
% In addition, it also sets the registers involved in the obfuscation operation during the analysis to be contaminated to determine the patching method to ensure that the original context is not corrupted.
% Due to the unknownness of obfuscating approach of the input, no matter functions are obfuscated by these two obfuscating approach or not, analysis flow will pass through this .


% \textbf{\textit{Flow Analyzer}} is the key step in the deobfuscation of control flow flatten. In this subsystem, classification of basic blocks will be first implemented to determine objects??? of subsequent symbolic execution. 
% The result of the symbolic execution will then dynamically adjust the order of basic block sequence to ensure the integrity of symbolic execution context. 
% We use Angr~\cite{shoshitaishvili2016state} as our symbolic execute engine due to its outstanding accuracy and performance on ARM platform. 

% \textbf{\textit{Re-builder}} is responsible for patching the binary,
% which obfuscated by instruction substitution and bogus control flow, 
% rebuilding and optimizing (i.e. the split blocks connected by direct jump are merged together) the control flow graph of a flattened function. It is also responsible for removing dead blocks when bogus control flow mixed with control flow flatten.
%  introduced by bogus control flow 

Next, we will elaborate on the details of \Name and how it works on each obfuscation technique in O-LLVM.


==> Automated Deobfuscation of Android Native Binary Code/Section4-InsSub.tex <==
\section{Instruction Substitution Deobfuscation}

The basic idea of InsSub is to replace standard binary operations by functionally equivalent but more complicated sequences of instructions. Note that in order to avoid the interference of constant folding~\cite{wiki:confold}, we set all variable as unknown numbers in our analysis, e.g. a variable waiting for user's input, in order to keep InsSub activated. Table~\ref{Tab:InsSubtable} summarizes 13 kinds of instruction substitution in 5 different categories, which are all the transformations we can find in O-LLVM. Among these transformations, three cases (which are highlighted in the table) are new and not specified in previous work~\cite{junod2015obfuscator}. 




\begin{table}[tbp]
    \centering

  \begin{threeparttable}
  \caption{Semantic features used in InsSub.}
  \vspace{-0.in}
  \label{Tab:InsSubtable}

    \begin{tabular}{c|c}
    \toprule
\multicolumn{1}{l}{Obfuscated Expression} & \multicolumn{1}{l}{Origin Expression} \cr
\midrule
{a = b - (-c)} &  \cr
{a = -(-b + (-c))} & \cr
{a = b + r; a += c; a -= r} & \cr
{a = b - r; a += c; a += r} & \multirow{-4}{*}{a = b + c}\cr
\midrule
{ a = b + (-c)} & \cr
 \textbf{\underline{a = -((-b) + c)}} &  \cr
a = b + r; a -= c; a -= r &  \cr
 a = b - r; a -= c; a += r & \multirow{-4}{*}{ a = b - c} \cr
\midrule
a = (b \(\oplus\) ! c) \& b &  \cr
{ \textbf{\underline{a = !(!b \(|\) !c) \& (r \(|\) !r)}}} & \multirow{-2}{*}{a = b \& c} \cr
\midrule
a = (b \& c) \(|\) (b \(\oplus\) c) & a = b \(|\) c \cr
\midrule
{a = (!b \& c) \(|\) (b \& !c)} & \cr
\textbf{\underline{a = (b \(\oplus\) r) \(\oplus\) (c \(\oplus\) r)}} & \multirow{-2}{*}{ a = b \(\oplus\) c} \cr
   \bottomrule
    \end{tabular}
    \end{threeparttable}
\end{table}



% on ARM platform, if the value of a variable was concrete, the InsSub will be optimized by NDK
% \haoyu{CITE HERE}
% \haoyu{Should describe the influence of this NDK optimization. Is is a challenge?}

%  \haoyu{bad presentation here. should discuss to find a better way.} \haoyu{Should describe why.}
% InsSub performs obfuscation on semantic level
\textbf{Challenges.}  
For each kind of operation, there are multiple ways to replace it with functionality equivalent instructions.
To achieve code diversification in the final results, the InsSub obfuscator randomly chooses one way to do the obfuscation. Besides, the obfuscated instructions are often interleaved with normal instructions (unobfuscated ones) at the assembly level, which is hard to separate. As a result, it is not enough by simply searching for specific opcode combinations during InsSub deobfuscation. 
Instead, we introduce static taint analysis to address this challenge.
% How to comprehensively and accurately recover these obfuscations has become a challenge for us.

% There are many alternatives for the obfuscator to choose randomly, and these obfuscations are often mixed with normal instructions at assembly level. As a result, the deobfuscation work is not simply lookup feature combination. How to comprehensively and accurately recover these obfuscations has become a challenge for us.

% 混淆器可供选择的替换方式非常多，并且这些混淆在汇编层面经常和正常指令混合在一起。所以，对于这种混淆恢复并不仅仅是简单的查找特征组合。如何对于这些混淆进行全面且精确地恢复，成为了我们的一大挑战


% is
% while the diversity of semantics and the randomness of instructions introduce challenges\haoyu{mark to do}.
% Also due to the optimization of ARM instructions, some obfuscation patterns may not be independent. Instead, they may rely on some instructions in the original semantics\lei{mangle}. 

% \subsubsection{Locate Features}

% % Our deobfuscation work on InsSub is based on semantic feature of assembly language \haoyu{may rewrite this sentence?}. 
% To identify code that use InsSub obfuscation, we have manually 
% summarized 11 kinds of features from 5 different categories, as discussed in paper~\cite{junod2015obfuscator}. 
% In addition, we also found a new obfuscating form (the highlight one) for subtraction during our analysis, which is not mentioned in original paper.
% \begin{table}[!htbp]
%     \centering
% %   \fontsize{6.5}{8}\selectfont
% % \resizebox{1\linewidth}{!}{

%   \begin{threeparttable}
%   \caption{Semantic Features used in InsSub}
%   \label{Tab:Benchmark:InsSubtable}

%     \begin{tabular}{c|c}
%     \toprule
%     \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}Obfuscated Expression} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}Origin Expression} \cr
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}a = b - (-c) \\ a = -(-b + (-c)) \\ a = b + r; a += c; a -= r\\ a = b - r; a += c; a += r\end{tabular}} & {\color[HTML]{333333} a = b + c} \cr
% \midrule
% \rowcolor[HTML]{EFEFEF} 
% \begin{tabular}[c]{@{}c@{}}a = b + (-c)\\ \textbf{\underline{a = -((-b) + c)}}\\ a = b + r; a -= c; a -= r \\ a = b - r; a -= c; a += r\end{tabular} & a = b - c \cr
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = (b \(\oplus\) !c) \& b} & {\color[HTML]{333333} a = b \& c} \cr
% \midrule
% \rowcolor[HTML]{EFEFEF} 
% a = (b \& c) \(|\) (b \(\oplus\) c) & a = b \(|\) c \cr
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% a = (!b \& c) \(|\) (b \& !c) & a = b \(\oplus\) a \cr
%    \bottomrule
%     \end{tabular}
%     \end{threeparttable}
    
% \end{table}

% \begin{table}[tbp]
%     \centering
% %   \fontsize{6.5}{8}\selectfont
% % \resizebox{1\linewidth}{!}{

%   \begin{threeparttable}
%   \caption{Semantic features used in InsSub.}
% %   \vspace{-0.1in}
%   \label{Tab:InsSubtable}

%     \begin{tabular}{c|c}
%     \toprule
%     \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}Obfuscated Expression} & \multicolumn{1}{l}{\cellcolor[HTML]{EFEFEF}Origin Expression} \cr
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b - (-c)} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = -(-b + (-c))} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b + r; a += c; a -= r} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b - r; a += c; a += r} & \multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} a = b + c}} \cr
% \midrule
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} a = b + (-c)} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} \textbf{\underline{a = -((-b) + c)}}} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} a = b + r; a -= c; a -= r} & \cellcolor[HTML]{EFEFEF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} a = b - r; a -= c; a += r} & \multirow{-4}{*}{\cellcolor[HTML]{EFEFEF}{\color[HTML]{333333} a = b - c}} \cr
% \rowcolor[HTML]{FFFFFF} 
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% a = (b \(\oplus\) ! c) \& b & \cellcolor[HTML]{FFFFFF} \cr
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} \textbf{\underline{a = !(!b \(|\) !c) \& (r \(|\) !r)}}} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}a = b \& c} \cr
% \midrule
% \rowcolor[HTML]{EFEFEF} 
% a = (b \& c) \(|\) (b \(\oplus\) c) & a = b \(|\) c \cr
% \midrule
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = (!b \& c) \(|\) (b \& !c)} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \cr
% \rowcolor[HTML]{FFFFFF} 
% \textbf{\underline{a = (b \(\oplus\) r) \(\oplus\) (c \(\oplus\) r)}} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} a = b \(\oplus\) c}} \cr
%   \bottomrule
%     \end{tabular}
%     \end{threeparttable}
    
% % \vspace{-0.15in}
% \end{table}

% \begin{table}[]
% \begin{tabular}{|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} Obfuscated expression} & {\color[HTML]{333333} origin expression} \\ \hline
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b - (-c)} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \\ \cline{1-1}
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = -(-b + (-c))} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \\ \cline{1-1}
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b + r; a += c; a -= r} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \\ \cline{1-1}
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = b - r; a += c; a += r} & \multirow{-4}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} a = b + c}} \\ \hline

% a = (b ˆ ! c) \& b & \cellcolor[HTML]{FFFFFF} \\ \cline{1-1}
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} \textbf{a = !(!b | !c) \&\& (r | !r)}} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}a = b \& c} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% {\color[HTML]{333333} a = (b \& c) | (b ˆ c)} & {\color[HTML]{333333} a = b | c} \\ \hline
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = (!a \& b) | (a \& !b)} & \cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} } \\ \cline{1-1}
% \rowcolor[HTML]{FFFFFF} 
% \textbf{a = (a \textasciicircum r) \textasciicircum (b \textasciicircum r)} & \multirow{-2}{*}{\cellcolor[HTML]{FFFFFF}{\color[HTML]{333333} a = a \textasciicircum b}} \\ \hline
% \end{tabular}
% \end{table}

% \begin{table}[htbp]
% \renewcommand\arraystretch{1.3}
% \centering
% \resizebox{0.8\columnwidth}{!}{
% \begin{tabular}{|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% \multicolumn{1}{|l|}{\cellcolor[HTML]{EFEFEF}Obfuscated Expression} & \multicolumn{1}{l|}{\cellcolor[HTML]{EFEFEF}Origin Expression} \\ \hline
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} \begin{tabular}[c]{@{}c@{}}a = b - (-c) \\ a = -(-b + (-c)) \\ a = b + r; a += c; a -= r\\ a = b - r; a += c; a += r\end{tabular}} & {\color[HTML]{333333} a = b + c} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% \begin{tabular}[c]{@{}c@{}}a = b + (-c)\\ \textbf{\underline{a = -((-b) + c)}}\\ a = b + r; a -= c; a -= r \\ a = b - r; a -= c; a += r\end{tabular} & a = b - c \\ \hline
% \rowcolor[HTML]{FFFFFF} 
% {\color[HTML]{333333} a = (b \(\oplus\) !c) \& b} & {\color[HTML]{333333} a = b \& c} \\ \hline
% \rowcolor[HTML]{EFEFEF} 
% a = (b \& c) \(|\) (b \(\oplus\) c) & a = b \(|\) c \\ \hline
% \rowcolor[HTML]{FFFFFF} 
% a = (!b \& c) \(|\) (b \& !c) & a = b \(\oplus\) a \\ \hline
% \end{tabular}}
% \end{table}



% In this step, Feature Extractor first detects whether any of the aforementioned semantic features exists, and then identifies the relationship among operands of these instructions \haoyu{mark to do}. If all conditions satisfied, Feature Extractor will regard the input as an obfuscated instruction sequence by InsSub \lei{modified by Lei}.

% 在这一步中，特征提取器首先会检测符合上述特征的指令组合是否存在，如果存在则认为函数使用了指令替换进行混淆。In this step, Semantical Feature Extractor will extract all matching instruction addresses that match the instruction replacement feature
% 在这一步中，特征提取器首先会检测上述特征的特征组合是否存在，如果存在则认为函数使用了指令替换进行混淆。

% \subsubsection{Taint Analysis}
\textbf{Method.}
We apply taint analysis to determine the combination of obfuscating instructions and locate instructions needed to be rewritten. 
% The analysis process of this subsystem is mainly divided into two steps. First is the opcode combination determining and then is the operands matching. 
We use the following example to illustrate how to use taint analysis to deobfuscate InsSub.

% Taint analysis is used to \Mark{mark to do}. 


%   MOV		R0, R4
  
%   BL		printf
  
%   ADD		R0, R7, R5
  
%   SUB		R6, R0, \#1
  
%   ADD		R0, R0, \#1
  
%   SUB		R7, R0, R5

%   B			loc\_8A0
  

% Lines 4,6 and 7 form a set of confusion for the addition operation.  
% It works with code simplification transformer to optimized the raw code. We use this code to discuss two different situations.
% \haoyu{mark todo}
% Taint Analyzer consists of two steps: opcode combination determining and operand matching. 

As shown in Fig.~\ref{insObfuscated}(a), assuming line 4 does not exist, the operations from line 3 to line 6 will lead to 
$R7 = R7 + R5 + 1 - R5 = R7 + 1$. After matching the opcode sequence $ADD, ADD, SUB$ and identifying the relationship between these operands, \Name will directly deobfuscate the assembly instruction sequence to its simplest form, $ADD R7, R7, \#1$. Finally, line 5 and line 6 will be replaced by NOP. 
% \lei{modified by Lei}

However, the existence of line 4 indicates that the value of $R6$ depends on $R0$. In this case, \Name will set the modified register $R0$ in line 3 as a tainted register. If there is an instruction operating with the tainted register between or after obfuscated instructions, the involved obfuscated instruction will be retained. As a result, instruction in Line 3 will be retained and instruction in Line 5 and 6 will be set as ``to be patched''. The tainted register will be freed after being modified by the follow-up instruction that is not related to this obfuscating procedure.

\lstset{language=c, label=inscon,
    basicstyle=\scriptsize\ttfamily,captionpos=b,escapeinside=``}
% {\begin{center}
% \vspace{-0.45in}
% \begin{minipage}[t]{1.03\linewidth}
% \begin{lstlisting}
% 	  case addr1:
% 		`\textbf{ToBoldThisLine((val\&0xF)!=(val|0xF), 1); }`
% 		....
% 	...}
%   }else{...}
% }
% \end{lstlisting}
% \end{minipage}
% \end{center}
% }

\begin{figure}
\centering
{\begin{minipage}{0.475\columnwidth}
\begin{lstlisting}[language={[x86masm]Assembler},basicstyle=\footnotesize]
---------------------
1 MOV	R0, R4
2 BL	printf
3 ADD	R0, R7, R5
4 SUB	R6, R0, #1
5 ADD	R0, R0, #1
6 SUB	R7, R0, R5
7 B	loc_8A0
---------------------
(a) Obfuscated
\end{lstlisting}
\end{minipage}}
{\begin{minipage}{0.475\columnwidth}
\begin{lstlisting}[language={[x86masm]Assembler},basicstyle=\footnotesize]
---------------------
MOV	R0, R4
BL	printf
ADD	R0, R7, R5
SUB	R6, R0, #1
`\textit{\textbf{ADD}}`    `\textit{\textbf{R7, R7, \#1}}`
`\textit{\textbf{NOP}}`
B	loc_8A0
---------------------
(b) Deobfuscated
\end{lstlisting}
\end{minipage}}
\vspace{-0.1in}
\caption{An example of InsSub deobfuscation.}
\vspace{-0.2in}
\label{insObfuscated}
\end{figure}


% \begin{figure}
% \centering
% \includegraphics[width=0.6\columnwidth]{approach_pic/BCF-new.png}
% \includegraphics[width=0.3\columnwidth]{approach_pic/BCF-re-new.png}
% \label{opaque}
% \caption{An Example of BCF Deobfuscation.}
% \end{figure}

% \begin{minipage}{0.5\columnwidth}
% \centering
% \begin{lstlisting}[language={[x86masm]Assembler},numbers=left,basicstyle=\footnotesize]
% obfuscated:		simplified:
% ---------------------- --------------------
% MOV	R0, R4		MOV	R0, R4
% BL	printf		BL	printf
% ADD	R0, R7, R5	ADD	R0, R7, R5
% SUB	R6, R0, #1	SUB	R6, R0, #1
% ADD	R0, R0, #1	ADD	R7, R7, #1
% SUB	R7, R0, R5	NOP
% B	loc_8A0		B	loc_8A0
% ---------------------- --------------------
% \end{lstlisting}
% \end{minipage}

% \subsubsection{Rewrite Binary}
% \haoyu{mark to do}
The deobfuscation result of InsSub is shown in Fig.~\ref{insObfuscated}(b). The content and address of the instructions that need to be modified will be saved temporarily and wait until other deobfuscating work finished, before rewritten to the binary.


==> Automated Deobfuscation of Android Native Binary Code/Section5-BCF.tex <==
\section{Bogus Control Flow Deobfuscation}


% \begin{figure*}[]
% \centerline{\includegraphics[width=0.3\textwidth]{pictures/BCF.png}}
% \caption{An example of Instruction Analyzer}
% % \vspace{-0.15in}
% \label{fig 2}
% \end{figure*}
% \includegraphics[scale=0.5]{BCF.png}
% \newline
BCF obfuscation introduces \emph{opaque predicates}\cite{wiki:opaque}
%\footnote{An opaque predicate~\cite{Opaque} is a predicate \(-\) an expression that evaluates to either ``true'' or ``false'' \(-\) for which the outcome is known by the programmer a priori, but which, for a variety of reasons, still needs to be evaluated at run time.} 
into the functions. 
The opaque predicate expression used in O-LLVM is \textbf{y\(<\)10 or (x*(x-1) mod 2)==0}. The second half of the expression is an odd number multiplying an even number modulo 2, which must equal 0. Hence, the whole expression will always be true, and the obfuscator introduces a dead branch to the code. Note that the branch will not be optimized by compilers due to the uncertainty of \textbf{x}. 
% \haoyu{no optimization}
% A dead branch consist of part of the content of the basic blocks in a real branch.  This is important for the deobfuscation of three pass mixed case, which will be illustrated in the Control Flow Flatten section.

\textbf{Challenges.} 
Although BCF obfuscation has \emph{modified} the control flow (by introducing dead branches), it is still instruction-level obfuscation. As a result, the challenge we encountered is similar to InsSub. However, BCF is significantly more complicated because the obfuscated instructions are often across basic blocks. To address this challenge, we also rely on taint analysis to perform global opaque predicate matching in order to remove dead branches efficiently.
% How to globally match opaque predicate operations has become a challenge for our deobfuscation work. 
% We still rely on taint analysis to address this challenge.
% \haoyu{mark to do. how and why?}
% \Mark{I already said in InsSub}

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.4\textwidth]{approach_pic/BCF-new.png}}
% \caption{BCF.}
% \vspace{-0.1in}
% \label{fig 4}
% \end{figure}
\begin{figure}[tbp]
\includegraphics[width=0.9\columnwidth]{approach_pic/bcf-new.pdf}
% \includegraphics[width=0.3\columnwidth]{approach_pic/BCF-after.png}
%%\vspace{-0.15in}
\caption{An example of BCF deobfuscation.}
\label{opaque}
\vspace{-0.1in}
\end{figure}

%  \haoyu{modify this figure.}
% \subsubsection{Determine Features}


% The principle of BCF is a pseudo-addition of control flow on the basis of instructions\haoyu{mark to do}. 

\textbf{Method.}
We rely on assembly features to detect whether a binary is obfuscated by BCF. 
For the given opaque predicate, we have summarized multiple assembly features. Note that InsSub may change the assembly features of BCF (e.g. sub operation may be obfuscated), thus we also manually summarized BCF features when InsSub is involved.

% Feature Extractor first extracts the initial control flow, and check the existence of assembly features of the opaque predicate operation. Once the feature was found, the input binary will be considered as obfuscated by BCF. 
% The initial control flow and all block contents \haoyu{mark to do} will be passed to Taint Analyzer.
% 事实上虚假控制流的原理也是在指令的基础上对控制流进行虚假的添加
% The initial control flow will first be extracted. Then, once the expression of the opaque predicate is determined, Feature Extractor is used to locate all basic blocks with opaque predicate operation \textbf{(x*(x-1) mod 2)==0}. It will save all addresses of these blocks in a list, and hooks all the registers which the opaque predicate changed the value of, to facilitate the follow-up taint analysis. 

% \subsubsection{Remove Bogus Branch}
% \subsubsection{Taint Analysis}
BCF introduces two branches to the original block using `CMP Rx, 0xA' (y$<$10). One successor block containing the `SUB MUL AND(S)' combination (maybe different implementations of the same expression `(x*(x-1) mod 2)' is used to direct the control flow back to the origin block. Another branch of this successor is always headed to a dead branch.
All basic blocks that take opaque predicates as jump conditions are designated as \textit{predicate blocks}. We use Fig. \ref{opaque} as an example to show how \Name works on this obfuscating pass. 
% \haoyu{mark to do. why use taint analysis and how.}

As shown in Fig. \ref{opaque} (1), the `SUB MUL ANDS' sequence first appears in \texttt{Block B}. When the opaque predicate operation is detected, taint analysis first sets \texttt{Block B} as a predicate block and sets R2 as a tainted register. Then it will force the conditional jump in the parent block reaching the predicate block \texttt{Block B}. After that, because only one condition jump of the predicate block can actually be accessed, taint analysis will head to \texttt{Block D} and label jump instruction at the end of \texttt{Block B} as to be modified. 
% The address of aimed alive block will be saved too to determine the actual modified instruction content.

Due to the optimization on ARM instructions during compilation, sometimes BCF obfuscation can occur as shown in \texttt{Block E}. If a conditional jump occurs and the constraint is a tainted register compared to zero (there are some cases that compare with 1), \Name will automatically set it as a predicate block. In this case, because register R2 is tainted, when system traverses the child blocks of \texttt{Block D}, the block \texttt{Block E} will be set as the predicate block too. The tainted register will be freed when modified by normal instructions.

% In subsequent analysis, if a conditional jump occurs and the constraint is a tainted register compared to zero (there are some cases that compare with one), Taint Analyzer will automatically set these blocks as predicate blocks. 

% Only the alive path will be explored in the follow-up process.
% Code simplification transformer will set instruction in Line 6 as the one that needs to be patched.
% The 'SUB MUL AND(S)' combination appears in the second block. As a result register R2 will be set as tainted register and No.2 and No.4 will be set as predicate blocks. Then it will first follow the conditional jump of 'CMP r1, \#A' to jump to the predicate block.

% In order to prevent instructions that affect original control flow from being destroyed, Taint Analyzer will let control flow pass through instead of avoiding predicate blocks. 

% \subsubsection{Rewrite Binary} 

After taint analysis, all deobfuscated information about instructions that need to be modified will be passed to the rebuilding process. When the binary is not obfuscated with CFF at the same time, the deobfuscated result (as shown in Fig. \ref{opaque} (2)) will be rewritten to the binary. 
% A simple deobfuscated result of BCF is shown in the right side of Fig. \ref{opaque}\haoyu{todo}. 
% After removing bogus branches and dead blocks, the original operation of this area is completely preserved.
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=0.4\textwidth]{approach_pic/BCF-re-new.png}}
% \caption{BCF.}
% \vspace{-0.1in}
% \label{fig 4}
% \end{figure}


==> Automated Deobfuscation of Android Native Binary Code/Section6-CFF.tex <==


\section{Control Flow Flattening Deobfuscation}

% The CFF obfuscation removes all easily identifiable conditional (e.g., \texttt{IF-ELSE}) and looping structures (e.g., \texttt{WHILE,FOR}), and reconstructs control flow through the use of a large \texttt{SWITCH} construct, which is responsible to route the code control flow through the proper basic blocks depending on a routing variable~\cite{junod2015obfuscator}.
% The dispatch process \haoyu{todo, rewrite}. 

The CFF obfuscation rebuilds the control flow to a \texttt{SWITCH} construct. To deobfuscate the control flow, we need to identify basic blocks that maintain original operations and rebuild the control flow. Symbolic execution is a means of using symbolic input to analyze a program to determine what inputs cause each part of a program to  execute~\cite{wiki:symbexe}. Since the analysis of CFF obfuscated code is flow sensitive, and symbolic execution has been proved as an effective program analysis technique that can systematically explore multiple program paths~\cite{cadar2011symbolic,anand2007jpf,cha2012unleashing}, we combine automatic static analysis and symbolic execution to deobfuscate the binary code. However, we still need to address the following \textbf{Challenges}: 


% Traditional static analysis is hard to explore the branches completely, while dynamic analysis typically are too complex to cover all the branches. \Mark{}
% Symbolic execution is a means of using symbolic input to analyze a program to determine what inputs cause each part of a program to execute~\cite{wiki:symbexe}. It has been proved as an effective program analysis technique that can systematically explore multiple program paths~\cite{cadar2011symbolic,anand2007jpf,cha2012unleashing}.
% \haoyu{cite 2-3 refs here}. 
% \haoyu{one sentence to introduce symexe here.}
% 由于ARM平台本身的优化特性，会对基本代码块

% \haoyu{why they are challenges? should describe more clear here.}\Mark{I wrote in each points}

% As a result, 

%%\vspace{-0.05in}
\begin{enumerate}
\item Due to the instruction optimizations introduced by the ARM compiler and obfuscator, original blocks are often split and reused. It is a challenge to identify the blocks that contain original operations from a super complicated control flow.
% How to identify basic blocks contain original operation from a super complicated control flow? 
% Identifying basic blocks contain original operation from a super complicated control flow. 

\item  As the original control flow has been destroyed by CFF, most basic blocks use direct jumps to reach successors after obfuscation. Before rebuilding the original control flow, we need to know what kind of blocks have multiple successors in the original flow. 

% How to determine the number of original successors of a obfuscated basic block is 
% Preforming context-aware symbolic execution. 

\item The recovery work on CFF-obfuscated code is flow-sensitive (e.g. the switch structure relies on the routing variable, which affects the control flow), thus we need to know how to maximize context inheritance and avoid path explosion.
% Due to the dependency of the switch structure on the routing variable, context information becomes very important in the recovery process. 
% flow sensitive 

\end{enumerate}
%%\vspace{-0.05in}
% We should maximize the context inheritance and avoid the problem of path explosion.
% \Mark{rewrite}

\Name first determines whether the code is obfuscated by CFF during preprocessing, and then conduct static analysis to identify basic blocks that contain original operations (\texttt{OO Blocks} for short). After that, it performs flow-sensitive symbolic execution on these blocks to reconstruct the original control flow. After optimization, the final deobfuscation result will be written to the output.

% we first use static analysis to find out basic blocks that contain original operations. Then symbolic execution is used to recover jumps between these basic blocks.

% XXX Then XXX...\haoyu{summarize the CFF Deobfuscation approach here.}

\subsection{Feature Extraction}
% The first step of our deobfuscation system is to make sure whether a function is obfuscated by CFF, which will be achieved by Feature Extractor. 
Since the flow between basic blocks is directed by a big switch construct, which is led by a routing variable, we use this switch construct and routing variable as two fingerprints to identify CFF-based obfuscation. 
% Based on manually analysis, we found that t
% \texttt{IF-ELSE} 
% After determining CFF is used to obfuscate code, Feature Extractor will extract 

The switch construct is actually a nested set of conditional jumps. As shown in Fig. \ref{CFF Structure}, each block ending with a conditional jump mainly consists of three instructions. We call these blocks \textbf{Dispatchers}. Also, the second operand of the compare instruction, which is different from other compare operations, is determined by both the value of the ARM \textbf{R15} register (Program Counter Register) and an immediate number \(\alpha\). \Name calculates the value of routing variable as follows:
\begin{equation}
V_{routing}=\alpha+ ins.address + 8\label{con:routine}
\end{equation}

% \textbf{routing variable =} \textbf{\(\alpha\)} \textbf{+ instruction.address + 8}

% \footnote{In Thumb mode, the value of PC Register equals current instruction address add 4.}
Here, \texttt{ins.address} is the address of the current instruction, which will be added by 8 (add 4 in Thumb mode), and becomes the value of Register R15 in the ARM mode.
All values of \(V_{routing}\) are saved into a dispatcher dictionary. 
%  which we called \textbf{\textit{KEY DICT}}


\subsection{Identification the OO Blocks}

Though CFF ruined the original control flow, original operations still exist in part of the obfuscated basic blocks. 
To re-construct the control flow, we first need to identify the \texttt{OO Blocks}, i.e., the blocks containing the \textbf{\textit{Original Operations}}.
In reference to previous work on the x86 platform~\cite{gabriel2014deobfuscation}, and combined with the characteristics of CFF on ARM, we divided the obfuscated control flow structure into five categories, as shown in Fig. \ref{CFF Structure}.

\begin{figure}[tbp]
\centerline{\includegraphics[width=0.5\textwidth]{approach_pic/cff-new.pdf}}
\vspace{-0.1in}
\caption{An example of a CFF obfuscated function.}
\vspace{-0.2in}
\label{CFF Structure}
\end{figure}

\textbf{Prologue} is the entrance block that contains information about almost all the constants in the original function. 

\textbf{Dispatcher} is a conditional-jumping block whose constraint is determined by R15 and an immediate number.
% which contain elements in KEY DICT. 

\textbf{Pre-dispatcher} is the Dispatcher block whose in-degree is larger than two. Note that an obfuscated function may have more than one Pre-dispatchers. 
% It is often same as the return block of the unobfuscated function. 

\textbf{Return} is the basic block whose out-degree is 0. Note that an obfuscated function may have more than one Return blocks.
% The search for Relevant blocks is the most important thing in the entire deobfuscating process, and it decides the correctness of the following-up work.

\textbf{Relevant} is the basic block that maintains operations of the original function. 
\Name does a reverse traversal from the Pre-dispatcher until it encounters a Dispatcher block. All basic blocks in this path between the Pre-dispatcher and Dispatcher are Relevant blocks because these blocks are all dispatched by the switch structure.

The original operations exist in Prologue, Return and Relevant Blocks, which forms the \texttt{OO Blocks}. 
Due to the introduced optimizations,  Relevant blocks may be partly merged, as the bottom gray block shown in Fig. \ref{CFF Structure}. In this case, the block will be duplicated and added to its two parent nodes.
% Taint Analyzer does a reverse traversal from the Pre-dispatcher until it encounters element in Dispatchers. In these resulting paths, all basic blocks between the Pre-dispatcher and Dispatcher are Relevants. Due to the optimization on ARM, some Relevants may partly merged, as the gray block in Figure.\ref{CFF Structure}. In this case, gray block will be duplicated and added to its two parent nodes.

%  a Relevant block has multiple branches or not
\textbf{Determine the number of original successors.}
Before the recovering process, we need to determine whether an \texttt{OO Block} has multiple successors when it was in the original control flow. 
% Note that Prologue block has one or two branches, ASSUME. \haoyu{todo here} Thus, we only need to analyze the Relevant blocks. 
The goal of this step is to prepare for subsequent analysis. Symbol execution will be performed twice to explore each possible path if a basic block has two successors.
% \haoyu{rewrite}

% Once a Relevant block has instruction which assigns a register, and the second operand of this instruction is dependent on R15 register, we calculate the result use Formula.\ref{con:routine}. If the calculation result exists in the range of dispatcher dictionary

Different from previous work on the x86 platform~\cite{gabriel2014deobfuscation}, which just used the opcode `CMOV' as the feature to detect the existence of multiple branches, and due to the simplicity of the ARM instruction set, we use elements in the previously mentioned dispatcher dictionary as the main indicator. If the second operand of an assignment operation exists in the dispatcher dictionary, the assigned register will be set as ``tainted register''. If there is a tainted-register-involved conditional move instruction on the path of this block back to Pre-dispatcher, we consider that this block has multiple successors in the original control flow. As previously mentioned, the tainted register will be freed when modified by a normal instruction. As shown in Fig. \ref{CFF Structure}, the yellow block (loc\_820) is an example that has two branches in the original function. 

% In this block, there is an instruction 'LDR R1, [R15, \#0x118]' and the calculation result of \textbf{formula 1} exists in dispatcher dictionary. As a result, R1 will be set as a taint register. Also there is a conditional move instruction 'MOVNE R1, R9' on the path the flow go back to Pre-dispatcher, which involves the taint register R1. According to our theory, this highlight basic block will be judged having two branches.



\subsection{Flow-sensitive Symbolic Execution}

Symbolic execution can be used to systematically explore multiple program paths\cite{trabish2018chopped}. 
However, due to unknown path constraints of the obfuscated program, directly applying symbol execution to explore all possible branches will cause path explosion.
% if the symbol execution is directly performed, it is easy to cause the path explosion problem. 

\subsubsection{Chopped Symbolic Execution}

\mbox{} \\ Inspired by the theory of chopped symbolic execution by David \textit{et.al}~\cite{trabish2018chopped}, which mainly targeted the exploration to paths of importance, we decide to separate the process of symbolic execution and set each \texttt{OO Block} as an object to be analyzed. For each basic block that needs to be analyzed, if it is previously determined to have two successors, symbolic execution will be performed twice to find out each of its successors separately. Otherwise the execution will be performed only once.
% 对于每个需要分析的基本块，我们会对其每个后继分别进行查找。如果一个基本块之前被判定存在两个后继，则对他的符号执行将会进行两次。
We use Angr~\cite{shoshitaishvili2016state} as our symbolic execution engine to perform symbolic execution on each \texttt{OO Block} in turn. 

% Here, }, a XXXX tool\haoyu{todo here} .

% In fact, Dispatcher and Pre-dispatcher blocks are added by the obfuscator to build the switch construction. Basic blocks which are useful for our recovery work exist in Prologue, Relevants and Return. We set each useful basic block as analysis object and perform symbolic execution on them in turn. 

% 子标题要改
% 一段保留，2过程
% \item \textbf{The order of symbolic execution.}\newline
% In fact, Dispatcher and Pre-dispatcher blocks are added by the obfuscation tool to build the switch construction. Basic blocks which are useful for our recovery work exist in Prologue, Relevants and Return. 

\subsubsection{Execution Process}

\mbox{} \\ \Name first pushes Relevant blocks into a block sequence. Initially, these blocks are out of order. The Prologue block is the first one to be analyzed. Note that in \Name, we always assume that Prologue has two succeeding branches. As a result, \Name performs symbolic execution twice on Prologue to explore both branches. We use the break point function in Angr to interrupt the execution before conditional \texttt{move} instructions. By changing the execution state, it will let control flow enter both True and False branches.
% \haoyu{explain why} 
% add \texttt{BP\_BEFORE} type breakpoint to the \texttt{statement} attribute. 
%  and execute the action function we set. When the symbolic execution is interrupted
% \texttt{claripy.BVV(1,1)}
% \texttt{claripy.BVV(0,1)}
% Here \texttt{claripy.BVV(v, len)} creates a \textbf{\textit{len-bit}} vector with the value of \textbf{\textit{v}}. 

When the execution stops before the break point, our system will set the conditional flag in Angr's Intermediate Representation to symbol 0 and 1, respectively, for the purpose of exploring its both following branches. For blocks with a single branch, \Name does not modify the state and analyzes them directly. The symbolic execution will keep stepping on until reaching an element in the block sequence or Return. 

% As a result, before the execution, our system will firstly traverse each instruction in this basic block and its son blocks.
\subsubsection{Cross-Function Protection}

\mbox{} \\ During symbolic execution, it is possible to enter another function's space through the function call. In ARM instructions, calling functions are done via \texttt{`BL'} or \texttt{`BLX'}. \Name hooks these two call instructions. When symbolic execution encounters hooked addresses, it will automatically skip the call instruction and continue the analysis in the space of the current function.

% todo
{
\begin{algorithm}
\caption{Dynamic Queue Scheduling Algorithm.}
\LinesNumbered %要求显示行号
\KwIn{Prologue \textit{P}, Relevants \textit{R}, Return \textit{Q}}%输入参数
\KwOut{Recovered control flow \textit{F}}%输出

    BlocksQueue[0] = \textit{P}\;
    BlocksQueue[1: ] = \textit{R} + \textit{Q}\;
    % OO\_Blocks = Prologue + Relevants + Return\;%\;用于换行
    Swap\_Pointer $\Leftarrow$  BlocksQueue[1]\;
    
    % successor1, CurrentState1 = SymbExec (Prologue, flag=true)\;
    % SavedState[successor1] = save (CurrentState1)\;
    % F[Prologue] = F[Prologue] + successor1\;
    
    % successor2, CurrentState2 = SymbExec (Prologue, flag=false)\;
    % SavedState[successor2] = save (CurrentState2)\;
    % F[Prologue] = F[Prologue] + successor2\;

    % Execution\_Pointer = BlocksQueue[0].address\;
    % swap(successor1, 

\For{i \textbf{in} range(0: len(BlocksQueue))}{
    BB = BlocksQueue[i]\;
    \eIf{BB has saved\_state}{
        RecoverState(SavedState)\;}
        {RecoverState(BlankState)\;}
    
    successor\_num = find\_branch(BB)\;

        \eIf{successor\_num == 1}{
            successor, CurrentState = SymbExec (BB, flag=None)\;
            SavedState[successor] = save (CurrentState)\;
            \textit{F}[BB].successor += successor\;
		\If{successor.address > Swap\_Pointer}
			{
			    swap(successor, Swap\_Pointer)\;
			    Swap\_Pointer++\;
			}
        }{
            successor1, CurrentState1 = SymbExec (BB, flag=true)\;
            SavedState[successor1] = save (CurrentState1)\;
            \textit{F}[BB].successor += successor1\;
            \If{successor1.address > Swap\_Pointer}
			{
			    swap(successor1, Swap\_Pointer)\;
			    Swap\_Pointer++\;
			}
            
            successor2, CurrentState2 = SymbExec (BB, flag=false)\;
            SavedState[successor2] = save (CurrentState2)\;
            \textit{F}[BB].successor += successor2\;
            \If{successor2.address > Swap\_Pointer}
			{
			    swap(successor2, Swap\_Pointer)\;
			    Swap\_Pointer++\;
			}
        }
    }

\Return{\textit{F}}
\end{algorithm}
}

\begin{figure}[t]
\centerline{\includegraphics[width=0.5\textwidth]{approach_pic/Symbexe.pdf}}
\vspace{-0.1in}
\caption{An example of dynamic queue scheduling.}
\vspace{-0.3in}
\label{fig:Symbexe}
\end{figure}

% \begin{figure}[htbp]
% \begin{minipage}[htbp]{\linewidth}

% \textcircled{1} \textit{Symbolic execution of Prologue for \textbf{True} branch}

% \textcircled{2} \textit{Swap returned Block 5 with the first block. Save context}

% \textcircled{3} \textit{Move Swap Pointer}

% \textcircled{4} \textit{Symbolic execution of Prologue for \textbf{False} branch}

% \textcircled{5} \textit{Swap returned Block 3 with the second block. Save context}

% \textcircled{6} \textit{Move Swap Pointer}

% \textcircled{7} \textit{Move Execution Pointer}


% \end{minipage}%

% \end{figure}

% \haoyu{rename}
% context-aware
% As illustrated in \textbf{figure}, assuming that two times symbolic execution of Prologue return two different addresses, it proves that there are two branches in the end of this block. We use symbol \(B_{1}\) and \(B_{2}\) to indicate two successor blocks respectively. Symbol \(S_{B_{i}}\) is used to indicate context state when the symbolic execution is executed to the start address of \(B_{i}\). Analyzer saves all \(S_{B_{i}}\) to a \textbf{\textit{STATE DICT}}. 

% After completing the symbolic execution of the Prologue block, Flow Analyzer advances the position of \(B_{1}\) and \(B_{2}\) to the forefront of block sequence \textbf{\textit{Q}}. A \textbf{\textit{Swap Pointer}} is used to indicate the last position that has been swapped. Then it performs symbolic execution on each block in Q successively with the approach described previously. Before each basic block being executed, our system looks in \textbf{\textit{STATE DICT}} for context information that it should recover. After restoring the context state, symbol execution will continue until the control flow passes through Pre-dispatcher and goes back to a basic block in \textbf{\textit{Q}}. If index of the returned basic block is after the position that variable \textbf{\textit{ind.}} points, the returned block will be swapped to the front of the unswapped position. After the complete analysis of each basic block, variable \textbf{\textit{ind.}} will increase by 1 to make sure its point position always behind the execution block.

% Performing symbolic execution in this way not only guarantees the context inheritance of each basic block, but also ensures the order of the entire analysis process.
\subsubsection{Flow-Sensitive Execution}

\mbox{} \\ Since there are dependencies between basic blocks in a function, the deobfuscation process is flow-sensitive. If the symbolic execution starting from each basic block uses a blank symbol state, it must cause basic block mismatching due to the loss of necessary context. 
% \haoyu{explain the challenge here} 
As a result, while performing symbolic execution on basic blocks, the deobfuscation system will dynamically save current execution state and adjust the position of the elements in block sequence to ensure the state inheritance. 
% they are \texttt{Execution Pointer} and \texttt{Swap Pointer}.

Two pointers are used in the process of symbolic execution: the \textit{Execution Pointer} pointing to the current analyzing block, and the \textit{Swap Pointer} pointing to the front position that never being swapped. Initially, the Execution Pointer points to the Prologue and the Swap Pointer points to the first block in the block sequence. The returned successor block will be swapped to the position that the Swap Pointer points to. At the same time, the current symbolic state will be saved. When the analysis proceeds to this successor, the saved state will be restored. If the returned successor block is before the Swap Pointer, there will be no exchange between basic blocks. But the symbolic state of this successor will be updated. After getting all successor block(s) of the current analyzing block, the Execution Pointer will move to the next block. In special cases when the two pointers coincide, \Name will move the Swap Pointer forward one space.

The purpose of dynamically exchanging basic blocks in the sequence is to ensure that most of the basic blocks inherit the state from the previous analysis before execution, while not starting the analysis of a basic block from a blank state. 

Algorithm 1 presents the top-level algorithm of our dynamic basic blocks scheduling approach. We also use Fig.~\ref{fig:Symbexe} as an example to show how this algorithm work. \textcircled{1} After analyzing the True branch, the state before executing Block 5 is saved. \textcircled{2} Then Block 5 is exchanged to the first place of sequence and \textcircled{3} the Swap Pointer is moved to the next. \textcircled{4} Following the analysis of the False branch, \textcircled{5} the successor Block 3 is swapped with the second block in sequence and \textcircled{6} the Swap Pointer is moved to the third position. At the same time the state reaching Block 3 will be saved. After that, \textcircled{7} the Execution Pointer points to the first block (Block 5) in the sequence and the previously saved state of Block 5 will be restored. The analysis of other blocks will continue like this successively.



% For blocks in the sequence that reached more than one time, the analyzer replaces the previous one with the latest context. And for very few basic blocks without a parent node, Flow Analyzer will restore the context that when Prologue reached Pre-dispatcher, and analyze these few blocks on this basis.



% After each time's symbolic execution, Flow 

% As illustrated in Figure.\ref{fig:Symbexe}, in the first time exploration of True branch, Flow Analyzer got one successor Block 5. A \textbf{\textit{Swap Pointer}} is used to indicate the newest position that to be swapped. Initially this pointer points to the head of sequence. Here because Block 5 is behind Swap Pointer, Analyzer will swap Block 1 and Block 5, then move Swap Pointer to the second position. To protect the context state and let the analysis go right, Analyzer will saves the current state of symbolic execution to a state dictionary. When the analysis proceeds to Block 5, the expected context state will be restored from the state dictionary.

% After the first part of analysis, symbolic execution of Prologue will be performed to explore the False branch. Analyzer got one successor Block 3. Because position of Block 3 is behind Swap Pointer, the same operation will be performed again. Now the first two in Block Sequence is Block 5 and Block 3, and Swap Pointer will point to the third position. When the whole analysis of Prologue finished, the Execution Pointer will be moved to the first position of the sequence. 

% If index of the returned basic block is before the position that Swap Pointer points, or is a Return Block, the returned block will not be swapped. After the complete analysis of one basic block, if positions of these two pointers are same, the Swap Pointer will increase by 1 to make sure its point position always behind the Execution Pointer.

% Then Flow Analyzer performs symbolic execution on each block in sequence successively with the approach described previously. Before each basic block being executed, our system looks in state dictionary for context information that it should recover. After restoring the context state, analysis of a block will continue until the control flow passes through Pre-dispatcher and goes back to one basic block in the sequence or in Return.

% The purpose of dynamically exchanging basic blocks in the sequence is to ensure that most of the basic blocks inherit the context information from the previous analysis before execution. For blocks in the sequence that reached more than one time, the analyzer replaces the previous one with the latest context. And for very few basic blocks without a parent node, Flow Analyzer will restore the context that when Prologue reached Pre-dispatcher, and analyze these few blocks on this basis.

Performing symbolic execution in this way not only guarantees the maximum state inheritance of each basic block, but also avoids path explosion and ensures the order of the entire analysis process. 

% \begin{figure}
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{approach_pic/anagram_before.png}
% \label{fig:side:a}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{approach_pic/anagram_after.png}
% \label{fig:side:b}
% \end{minipage}
% \caption{CFG merge Rule \uppercase\expandafter{\romannumeral1}}
% \end{figure}
% \begin{figure}
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{approach_pic/cmp_before.png}
% \label{fig:side:a}
% \end{minipage}%
% \begin{minipage}[t]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{approach_pic/cmp_after.png}
% \label{fig:side:b}
% \end{minipage}
% \caption{CFG merge Rule \uppercase\expandafter{\romannumeral2}}
% \end{figure}



% \textbf{Execution in the scope of current function.}
% For each basic block in sequence that needs to be analyzed, it is possible to enter the system's airspace or other functions through the function call. As a result, before the execution, our system will firstly traverse each instruction in this basic block and its son blocks. In ARM instructions, calling system functions or sub-functions is done via opcodes \textbf{'BL'} or \textbf{'BLX'}. Flow Analyzer will hook all these call instructions. When the symbol execution encounters hooked address, it will automatically skip call instruction and continue the execution in the airspace of the current function.

%  In the unobfuscated function, due to the reasonable arrangement of the compiler, there are few cases where a direct jump connection is used between multiple consecutive blocks. 


\subsection{Control Flow Reconstruction}
When using CFF to obfuscate the native code, there is a certain degree of basic block splitting and merging due to ARM optimizations, no matter the basic block splitting pass is activated or not. As a result, it is necessary to optimize the recovered control flow. We apply two optimization here.
% The optimization is mainly concentrated in two parts, as shown in Fig. \ref{fig:mergeRule}.

\uppercase\expandafter{\textbf{Rule \romannumeral1}}. As shown in Fig. \ref{fig:mergeRule} (1), for two nodes connected by a direct jump, if the in-degree of the parent node is not greater than one, \Name merges these two nodes.

\uppercase\expandafter{\textbf{Rule \romannumeral2}}. As shown in Fig. \ref{fig:mergeRule} (2), for multiple connected nodes, if their out-degree are all equal to two and the other branch of them points to a same node, once the contents of each node are alike (e.g. comparing operation with consecutive integers), \Name will optimize this structure as a loop.
% for multiple nodes with two branches, 
% if these nodes are connected in series by one branch, and their other branches point to the same node, once the opcode sequences are identified, 

Note that when BCF and CFF are used together (with or without InsSub), the introduction of opaque predicates does not affect the recovery of original control flow. Because these blocks (previous mentioned blocks in dead branch) are always unreachable, they will be removed in the final output.
\begin{figure}[htbp]
%\vspace{-0.2in}
\centering
\includegraphics[width=\columnwidth]{approach_pic/rule.png}
\vspace{-0.2in}
\caption{Control flow merging rules.}
\label{fig:mergeRule}
\vspace{-0.2in}
\end{figure}

% \section{Comprehensive Analysis of Real Situation}
% % 在现实中，由于输入函数的不确定性，我们并不知道该函数的混淆方式是哪一种。有可能是多种情况的混合，也有可能是没有进行混淆。所以这一部分我们会对该种情况进行说明
% In reality, due to the uncertainty of the input function, we don't know which obfuscation approach is used on it. There may be a mix of multiple passes, or there may be no obfuscation. So in this subsection we will discuss the real situation.

% For an input, the Feature Extractor first detects the obfuscated features of O-LLVM's three passes to determine which methods are used to obfuscate the function. In addition to the three individual cases mentioned above, there are four mixed cases:

% \uppercase\expandafter{\romannumeral1}. InsSub + BCF. In this case, features of the InsSub have not changed. The form of the BCF assembly instruction has changed, but the form of the opaque predicate operation is still (x*(x-1) \& 2)

% \uppercase\expandafter{\romannumeral2}. InsSub + CFF. In this case, the characteristics of two obfuscating methods do not affect each other.

% \uppercase\expandafter{\romannumeral3}. BCF + CFF. The feature determination in this case is dominated by the characteristics of CFF, and the useless blocks added by BCF do not affect the real control flow. The opaque predicate is still the feature of BCF. 

% \uppercase\expandafter{\romannumeral4}. InsSub + BCF + CFF. The features of the InsSub have not changed. The other two obfuscating approaches' features are same as described in the previous point.
% % 1、IS+BCF 这种情况下两种特征没有发生变化，不透明谓词操作的形式依旧为x*(x-1)/2(汇编指令的形式发生了变化)
% % 2、IS+CFF 这种情况下，两种混淆方式的特征不会相互影响
% % 3、BCF+CFF 这种情况下，以CFF的特征为主，BCF添加的无用块不会影响真实的控制流
% % 4、IS+BCF+CFF 这种情况下IS的特征依旧独立，


% After determined what kinds of obfuscation are used, Taint Analyzer then works to locate obfuscation instruction of InsSub and BCF. Once the function is not obfuscated by CFF, the recover information will be sent to the Re-builder.

% If the CFF pass is activated even mixed with other obfuscation approaches, after taint analysis, the deobfuscating process will enter the Flow Analyzer to recover the origin control flow. Then the recover result of Taint Analyzer and Flow Analyzer will be used together in Re-builder to output the final deobfuscated result.

% It is worth mentioning that when BCF and CFF are used together (no matter with or without InsSub), the introduction of opaque predicates does not affect the recovery of the control flow. As opaque predicate is a key feature of the BCF, it is used to distinguish the dead block introduced by the obfuscator. This part of work is done in the Re-builder. The principle of distinction is that when there is a basic block X with an in-degree of 0 and it is not Prologue, a basic block containing X' s instructions and opaque predicate will be looked for in the vicinity of X in recovered control flow. If such a block exists, the basic block X will be removed.

% 值得一提的是，当BCF和CFF共同使用时（不管有没有使用IS），不透明谓词的引入并不会对控制流的恢复造成影响。而不透明谓词作为BCF的关键特征，用来区分引入的deadblock。这一部分的工作是在recover系统中完成的。区分的原则是，当存在入度为0且不是序言的基本块时，会在其恢复的控制流附近寻找包含其指令且含有不透明谓词的基本块。如果有这样的基本块存在，则将该入度为零的基本块（deadblock）移除。

% This part extracting semantical features from the original binary. Such as the 
% 对于输入的原始函数，Semantical Feature Extractor会先对其进行特征提取，包括指令和操作数层面和CF层面的，以判断该输入是否为ollvm混淆，并确定混淆手段是什么。之后，Semantical Feature Extractor会将这些后续工作所需要的信息传入Flow Analyzer

% This part mainly works to deobfuscate instruction substitution。我们针对ollvm的指令替换的5种模式，设计了

% \item \textbf{\textit{Taint Analyzer}} is mainly used to remove the obfuscation of instruction substitution and bogus control flow. It is responsible for discovering the general forms and variants of these two ways of obfuscation. Also it will set the instructions involved in the obfuscating operation in the analysis process as tainted to determine the patching approach to ensure the original context is not corrupted. 
% Due to the unknownness of obfuscating approach of the input, no matter functions are obfuscated by these two obfuscating approach or not, analysis flow will pass through this .


% \item \textbf{\textit{Flow Analyzer}} is the core part of the deobfuscation of control flow flatten. In this subsystem, classification of basic blocks will be first implemented to determine objects of subsequent symbolic execution. The result of the symbolic execution will then dynamically adjust the order of basic block sequence to ensure the integrity of symbolic execution context. We use Angr~\cite{shoshitaishvili2016state} as our symbolic execute engine due to its outstanding accuracy and performance on ARM platform. 

% \item \textbf{\textit{Rebuild System}} is responsible to patching the binary which obfuscated by instruction substitution and bogus control flow, rebuilding and optimizing(i.e. The split blocks connected by direct jump are merged together.) the control flow graph of a flattened function. 

% \section{Implement}

==> Automated Deobfuscation of Android Native Binary Code/Section7-Evaluation.tex <==
\section{Implementation and Evaluation}

% \subsection{Implementation}

% Our experiment is carry out on a machine with 2.9 GHz Intel Core i7 processor and 16 GB memory running macOS Version 10.13.6. When we did our research, the latest version of O-LLVM was 4.0, and all of our work was based on this version's obfuscator. It is noticeable that our approach is suitable for code that obfuscated by any OLLVM versions. 
Our experiment is based on O-LLVM 4.0, while our approach can be easily extened to code obfuscated by any OLLVM versions. We use Android NDK V16.1 to build shared libraries. The symbolic engine of DiANa is implemented based on Angr 7.8.2, which is inspired by existing work on x86 platform~\cite{CFFRef, CFFRef2}.
The function addresses are exported by IDA Pro 7.0.

\subsection{\textbf{Dataset}}

To evaluate the effectiveness of DiAna, we first need to build a reliable open source dataset with high coverage. We have applied our system to the following three different datasets, respectively. 

\textbf{C/C++ Obfuscation Benchmark.}
We first evaluate our system on a widely used C/C++ obfuscation benchmark~\cite{cbenchmarks}. This dataset was created to evaluate different obfuscation algorithms~\cite{banescu2016code}. It includes common basic algorithms, hash functions, and small programs (mainly containing combinations of \texttt{IF}, \texttt{WHILE}, and \texttt{FOR} structures). We eliminated the benchmark programs that contain only one basic block, because it is hard to apply obfuscation techniques on these tiny programs. At last, we obtain 94 benchmark programs in total to evaluate the effectiveness of DiANa.

\textbf{Open-Source Android Native Code.} 
To evaluate our system on real-world Android apps, we have crawled 100 open source Android projects from F-Droid~\cite{F-Droid}. Among them, 24 projects use native code. Note that Android apps could use native code in two ways: reusing the existing native libraries by embedding the $*.so$ in the project or implementing their own C/C++ code and then compiling it within the project. Finally, we have identified 5 real-world Android projects that contain open source C/C++ code, which can be used to evaluate our approach. 

\textbf{Real-world Andrioid Root Exploit.} 
We further apply \Name to Android Root Exploits (aka REs), a binary tool used to obtain the root privilege by exploiting privilege escalation vulnerabilities. In this case, we could evaluate the effectiveness of \Name on deobfuscating real threats in the wild.

% As many malware may hide the malicious payload in the native code to evade detection, we found a real-world malware case that exploit the towelroot vulnerability to XXXX. 
% \Mark{TODODO DOD OODO DDOO DOD ODO}

%%\vspace{-0.05in}
\subsection{\textbf{Evaluation Metrics}}
We hereby define our evaluation metrics. We deployed \texttt{Euclidean Distance (ED)}, \texttt{Similarity of Control Flow Graph (Sim)}, and  \texttt{Input/Output equivalence (I/O)} to evaluate the effectiveness and correctness of \Name.  Because InsSub works at the assembly instruction level and does not alter the control flow, we use \texttt{ED} to measure the deobfuscation effectiveness and \texttt{I/O} to ensure the correctness. For the BCF and CFF approaches, we deployed \texttt{Sim} to quantify the deobfuscation results, similar to previous work~\cite{yadegari2015generic}. Most importantly, we also use \texttt{I/O} to ensure the deobfuscated function is semantically equivalent to the original one. %Following is the detailed introduction to the three evaluation metrics.

\subsubsection{Euclidean Distance}
\mbox{} \\ 
We use Euclidean Distance as a quantitative indicator of our work on Instruction Substitution. To evaluate InsSub deobfuscation, we first generate a feature vector for each function. Each dimension in the vector represents the frequency of certain opcode. 
% We omit the details of calculating Euclidean Distance in this paper, which could be referred to.
We calculate the Euclidean distance~\cite{wiki:distance} as in Formula \ref{distance}.
\begin{equation}
d(x,y):=sqrt(\sum_{i=1}^{n}(x_i-y_i)^2)\label{distance}
\end{equation}

Here, $x$ and $y$ are the feature vectors of the obfuscated/deobfuscated function and the original one respectively, while $n$ is the total number of types of opcode used in functions $x$ and $y$.

\subsubsection{CFG Similarity Comparison}

\mbox{} \\ 
From the perspective of reverse engineering, control flow analysis is an important procedure. Due to the difficulty of patching (rewriting) the CFF obfuscated native code at the assembly level, CFG analysis is a key technique in static analysis for Android apps. We adopted the algorithm of Hu~\cite{hu2009large} for computing the edit distance between two CFGs, which was suggested as one of the best CFG comparison algorithms in previous empirical study~\cite{chan2014method}. It has also been widely used in previous work \cite{yadegari2015generic}\cite{pawlowski2016probfuscation}\cite{fyrbiak2018hybrid}.

The basic idea of this algorithm is to build a cost matrix that represents the costs of mapping different nodes in two graphs \textbf{\(G_1\)} and \textbf{\(G_2\)}. Then the Hungarian algorithm~\cite{kuhn1955hungarian} is used to find an optimal solution to the assignment problem in \(\mathcal{O}\)\((n^{3})\) time. Note that when calculating the similarity, we perform content matching (e.g. key API-call operation, instruction operands, etc) for each node. Although it does not perfectly prove that the deobfuscated semantics and the original semantics are completely equivalent, we believe that matching node content can further enhance the original similarity comparison algorithm, thus ensuring that the similarity value can reflect the accuracy of deobfuscation results to a certain extent.

We use the formula below to calculate the CFG similarity:
\begin{equation}
Sim(G_1,G_2) = 1-\frac{\sigma(G_1,G_2)}{|N_1|+|N_2|+|E_1|+|E_2|}\label{CFGSim}
\end{equation}

Here, \textbf{\(\sigma(G_1,G_2)\)} represents the edit distance between \(G_1\) and \(G_2\), \(|N_i|\) is the number of nodes in \(G_i\), and \(|E_i|\) is the number of edges in \(G_i\). The score given by Pearson correlation~\cite{pearson1896mathematical} is in the range of [-1,1]. The closer the score is to 1, the more similar are the structures of these two graphs. A similarity score less than 0 means that two graphs are completely dissimilar~\cite{chan2014method}. 



% Previous work suggested that after obfuscation, the CFG similarity score is roughly 0.2, while
% the CFG similarity score achieves higher than 0.8 after deobfuscation is a promising result.

\subsubsection{Semantic Equivalence}
\label{sec:semantic}
\mbox{} \\ 
Though we adopt strict block matching in the calculation of CFG similarity, it is not convincing enough to prove that the deobfuscated function is semantically equivalent to the original one. 
%%In other word, even a CFG similarity value is 1.0, we should also prove the correctness of our deobfuscation result. 
Due to the change of the offset and function size, binary rewriting needs to be performed on each subsequent instruction and function from the $*.so$ file, which may bring disturbances to the deobfuscation result. Also, to the best of our knowledge, there is no effective and accurate way to solve the problem of binary rewriting yet, even from the intermediate representation level. To minimize the introduction of bias caused by other tools, we choose to show our deobfuscation result of the CFF method on the disassembly instruction level, which is useful for reverse analysts to analyze malicious apps.


Regarding correctness, after applying deobfuscation, we use Angr's bit vector to generate 1,500 concrete value inputs (the 500 smallest integers, the 500 largest ones, 500 random others) and test whether the two corresponding outputs (origin and deobfuscated) are identical. If yes, we consider the deobfuscated code as semantically equivalent to the original one. We use \texttt{Input/Output equivalence (I/O)} to represent this evaluation process, which has also been widely used in previous work\cite{salwan2018symbolic}. In order to visualize the experimental results, we use the percentage of the identical I/O in 1500 times of experiments as a quantitative indicator. 


% 这里考虑两种方法，一是比较每个基本块的匹配程度，二是比较同样输入的输出的一致性。

%  with 1 indicating total positive correlation, 0 indicating no correlation, and -1 indicating negative correlation. In another word, 
% After completing the comprehensive deobfuscation analysis on the open source C benchmark, we look into the deobfuscating accuracy of our approach on Open Source Android Native Code. We evaluate the accuracy of our deobfuscating approach of BCF and CFF on functions in these binaries.

\subsection{\textbf{Evaluation on C/C++ Obfuscation Benchmarks}}

% \haoyu{First, detailed describe the dataset.}

% \haoyu{for each pass, (1) one paragraph to summarize the result (2) one paragraph to describe one case (better to show the good one) (3) one paragraph to explain the outliers}

Because InsSub only works on computation-intensive programs, we select 5 programs with many computation-related instructions from the benchmark to evaluate the result of InsSub deobfuscation. 

For BCF and CFF, we apply them to all the 94 programs in the benchmark and use \Name to deobfuscate them. We classified the benchmark programs into 5 categories based on their main functionalities: (1) sorting algorithm (Sort), (2) searching algorithm (Search),(3) mathematical calculation (Math), (4) string manipulation (String) and (5) conversion between number and string (Num2String). Furthermore, we also evaluated \Name on cases when all three obfuscation techniques are applied.

% For the source code in the small programs folder, we classify them according to their program structure. In addition, five source codes in the small program folder are too simple (i.e. the unobfuscated function has only one basic block), so we did not make analysis on them. 


\subsubsection{Instruction Substitution}
\mbox{} \\ 
The five programs used in the evaluation include: (1) Binary search, (2) Merge sort, (3) String splicing operation, (4) Quicksort and (5) a program with five arithmetical operations. For these programs, we first apply InsSub to obfuscate the samples and then use \Name to deobfuscate them. Note that for the pass of instruction substitution, we could deobfuscate the results to the binary level.

% The result is shown in Table~\ref{Tab:Benchmark:InsSubtable}. 
\textbf{Euclidean Distance.}
Column 2 and 3 in Table~\ref{Tab:Benchmark:InsSubtable} list the Euclidean distance between the obfuscated function and the unobfuscated one (\(D_{ob}\)), and between the deobfuscated one and the unobfuscated one (\(D_{de}\)), respectively. 
% The smaller the value, the more similar the instructions. 
As we can see, distances between obfuscated functions and unobfuscated ones are in the range of 14 to 44. After deobfuscation, the distances of the recovered functions are all below 10. Note that the gap between deobfuscated and unobfuscated binary (\(D_{de}\)) is mainly caused by the assignment of registers and memory addresses, e.g., \texttt{move}, \texttt{load} and \texttt{store} operations. 
% , when there are relatively more calculation operations in the source code, the obfuscated and the unobfuscated binary have a relatively larger gap at the instruction complexity\haoyu{suggest cut this sentence}. 

\textbf{The number of obfuscated operations.}
We also manually checked the obfuscated and deobfuscated programs to measure the number of obfuscated operations (\(N_{ob}\)) introduced and the number of operations (\(N_{de}\)) successfully recovered, as listed in Column 4 and Column 5 in Table~\ref{Tab:Benchmark:InsSubtable}. All the obfuscated operations are successfully recovered to binary files in our experiment. 

\textbf{Semantic Equivalence.}
We then applied the aforementioned approach (Section~\ref{sec:semantic}) to evaluate the semantic equivalence of deobfuscated binaries and the original ones. As shown in the \textit{``SE''} column of Table~\ref{Tab:Benchmark:InsSubtable}, for each program, we get identical outputs for all the 1500 generated inputs, suggesting that the deobfuscated binaries are semantically equivalent to the original ones.
%%Also the deobfuscated binary files are proved to be semantic equivalent to the original ones by the previous mentioned \texttt{I/O} approach(Column \textit{``SE''}).
% In addition, the function of the recovered binary is also preserved intact\haoyu{To be modified}.
% Also we verified the correctness of the function recovery
%   And the gap between deobfuscated and unobfuscated binary is mainly caused by the assignment of registers and memory addresses, such as move and load operation. 


\begin{table}[t]
    \centering
%   \fontsize{6.5}{8}\selectfont

  \begin{threeparttable}
  \caption{InsSub deobfuscation result.}
  \vspace{-0.1in}
  \label{Tab:Benchmark:InsSubtable}
    \begin{tabular}{c|ccccc}
    \toprule
    Name&\(D_{ob}\) & \(D_{de}\) & \(N_{ob}\) & \(N_{de}\) & SE
    \cr
    \midrule
    binarysearch & 17 & 9 & 5 & 5 & 100\% \cr
    mergesort & 16 & 8 & 2 & 2 & 100\% \cr
    concatstrings & 22 & 0 & 3 & 3 & 100\% \cr
    quicksort & 14 & 3 & 2 & 2 & 100\% \cr
    basic\_arithmetic\_operators & 44 & 10 & 8 & 8 & 100\% \cr
   \bottomrule
    \end{tabular}
      \vspace{-0.2in}
    \end{threeparttable}

\end{table}


% \begin{table}[!htbp]
% \caption{InsSub Result}
% \label{Tab:Benchmark:InsSubtable}
% \renewcommand\arraystretch{1.5}
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|}
% \hline
%  & \cellcolor[HTML]{C0C0C0}\(D_{obf}\) & \cellcolor[HTML]{C0C0C0}\(D_{deobf}\) & \cellcolor[HTML]{C0C0C0}\(Num_{obf}\) & \cellcolor[HTML]{C0C0C0}\(Num_{deobf}\) \\ \hline
% {\color[HTML]{343434} binarysearch} & 17 & 9 & 5 & 5 \\ \hline
% {\color[HTML]{343434} mergesort} & 16 & 8 & 2 & 2 \\ \hline
% {\color[HTML]{343434} concatstrings} & 22 & 0 & 3 & 3 \\ \hline
% {\color[HTML]{343434} quicksort} & 14 & 3 & 2 & 2 \\ \hline
% {\color[HTML]{343434} basic\_arithmetic\_operators} & 44 & 10 & 8 & 8 \\ \hline
% \end{tabular}}
% \end{table}

% The confusing meaning of instruction substitution is very weak, it only makes troubles for the analyst to understand the function in the calculation part. As a result, our deobfuscation work is only for the official default obfuscation setting, that is the case where obfuscation loop is one.



% We selected four computationally intensive algorithms from the open source benchmark. In addition, we have written a program which contains five operations that obfuscator aimed in instruction substitution. 
% we calculate both the Euclidean distance between the obfuscated function and the unobfuscated one(\(D_{obf}\)), and the Euclidean distance between the deobfuscated one and the unobfuscated one(\(D_{deobf}\)). The results are shown in Table. \ref{InsSubtable}. The smaller the value of \(D_{A\_to\_B}\) is, the more similar instructions of function A and function B are. In addition, the number of obfuscated operation(\(Num_{obf}\)) and the number of recovered operation(\(Num_{deobf}\)) are also given in the table.

% \begin{figure}
% \begin{minipage}[htbp]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{pictures/ins.png}
% \label{fig:side:a}
% \end{minipage}%
% \begin{minipage}[htbp]{0.5\linewidth}
% \centering
% \includegraphics[width=0.5\linewidth]{pictures/ins-re.png}
% \label{fig:side:b}
% \end{minipage}
% \caption{CFG merge Rule \uppercase\expandafter{\romannumeral1}}
% \end{figure}

% \haoyu{TODO this paragraph}

% To evaluate the effectiveness of instruction substitution deobfuscation, 
% we firstly selected four computationally intensive source code and applied our deobfuscating approach on them. After that, we made deobfuscation of control flow flatten and bogus control flow on function of this dataset separately. Also, to illustrate the accuracy of our approach, we use both the default settings and enhanced settings on both obfuscation passes. Then the three-passes-mixed situation is evaluated too. 



\subsubsection{Bogus Control Flow}
\mbox{} \\ 
BCF offers two additional obfuscation options \texttt{bcf\_loop} and \texttt{bcf \\ \_prob}, which controls the obfuscation times (default 1) and obfuscation intense (default 30\%).
To evaluate the effectiveness of \Name on BCF deobfuscation, we applied two different levels of obfuscation intense: the default obfuscation (bcf\_prob=30\%), and enhanced obfuscation (bcf\_prob=50\%). We are also able to recover the deobfuscated code to the binary level.
% They are situations of default and bcf\_prob=50\% respectively. 


\textbf{Result.}
Table~\ref{table:opencresult} shows the overall result. 
Column \textit{``BCF''} and Column \textit{``BCF\_re''} shows the result at the default obfuscation level, and Column \textit{``BCF\_50\%''} and Column \textit{``BCF\_50\%\_re''} shows the result of the enhanced one. 
At the default level, the CFG similarity between the original program and the obfuscated program is 0.453 on average, while the CFG similarity could reach up to an average of 0.870 after the deobfuscation process. 
For the enhanced obfuscation, CFG similarity score of most obfuscated functions has a significant decrease, with an average score of 0.296. Nevertheless, our system could achieve similar good results at different obfuscation level, with an average CFG similarity score of 0.855.

{\begin{table*}[ht!]

\caption{Deobfuscation results on the C/C++ Benchmark.}
%%\vspace{-0.1in}
    \centering
  \fontsize{6.5}{8}\selectfont
\resizebox{1\linewidth}{!}{
  \begin{threeparttable}
%\setlength{\tabrowsep}{1pt} % Default value: 6pt
\renewcommand{\arraystretch}{} % Default value: 1  
    \begin{tabular}{c|ccc|ccc|ccc|ccc|ccc}
    \toprule
    Name & BCF & BCF\_re  & SE & BCF\_50\% & BCF\_50\%\_re & SE & CFF & CFF\_re & SE & CFF-3 & CFF-3\_re & SE & ALL & ALL\_re & SE 
    \cr
    \midrule

selectionsort & 0.904 & 0.938 & 100\% & 0.398 & 0.938 & 100\% & 0.151 & 0.910 & 100\% & -0.160 & 0.875 & 100\% & -0.128 & 0.747 & 100\% \cr
 
bubblesort & 0.709 & 0.852& 100\%  & 0.469 & 0.970& 100\%  & 0.200 & 0.818& 100\%  & -0.160 & 0.726& 100\%  & -0.230 & 0.821& 100\%  \cr
 \midrule
 
binarysearch & 0.759 & 0.897& 100\%  & 0.372 & 0.923 & 100\% & 0.137 & 0.868 & 100\% & -0.192 & 0.868 & 100\% & 0.023 & 0.816 & 100\% \cr
 
binarysearchrec & 0.597 & 0.750 & 100\% & 0.326 & 0.750 & 100\% & 0.318 & 0.843 & 100\% & -0.130 & 0.816 & 100\% & 0.023 & 0.816 & 100\% \cr
 \midrule
 
gcd & 0.660 & 0.872 & 100\% & 0.388 & 0.872 & 100\% & 0.075 & 0.776 & 100\% & -0.211 & 0.776 & 100\% & -0.294 & 0.776 & 100\% \cr
 
 lcm & 0.152 & 0.912 & 100\% & 0.365 & 1.000 & 100\% & 0.172 & 0.857 & 100\% & -0.218 & 0.912 & 100\% & -0.218 & 0.912 & 100\% \cr
 \midrule
 
 concatstrings & 0.213 & 0.769 & 100\% & 0.133 & 0.795 & 100\% & 0.213 & 0.778 & 100\% & -0.261 & 0.872 & 100\% & -0.124 & 0.872 & 100\% \cr
 
 reverse & 0.280 & 1.000 & 100\% & 0.370 & 0.900 & 100\% & 0.292 & 0.926 & 100\% & -0.252 & 0.828 & 100\% & -0.114 & 0.828 & 100\% \cr
 \midrule
 
 romannumerals & 0.234 & 0.797 & 100\% & 0.321 & 0.816 & 100\% & 0.164 & 0.797 & 100\% & -0.250 & 0.869 & 100\% & -0.340 & 0.807 & 81\% \cr
 
 decimaltobinary & 0.184 & 0.906 & 100\% & 0.253 & 0.783 & 100\% & 0.310 & 0.854 & 100\%  & -0.174 & 0.854 & 100\% & 0.016 & 0.854 & 100\% \cr
 \midrule
 
 bkdrhash & 0.175 & 0.828 & 100\% & 0.155 & 0.822& 100\% & 0.294 & 0.926 & 100\% & -0.165 & 0.828 & 100\% & -0.070 & 0.926 & 67\% \cr 
 
 djbhash & 0.378 & 0.828 & 100\% & 0.409 & 0.813 & 100\% & 0.264 & 0.926 & 100\% & -0.173 & 0.926 & 100\% & -0.198 & 0.742 & 100\% \cr
 \midrule
 
 \begin{tabular}[c]{@{}c@{}}1b-1-2-2-1-\\ gt127-0-0-0\end{tabular} & 0.618 & 1.000 & 100\% & -0.029 & 1.000 & 100\% & 0.304 & 1.000 & 100\% & -0.135 & 1.000 & 100\% & -0.126 & 1.000& 100\%  \cr
 \midrule
 
 \begin{tabular}[c]{@{}c@{}}1b-1-2-1-1-gtsum\\ 127\_dep-1-0-1\end{tabular} & 0.618 & 0.893 & 100\% & 0.083 & 0.737 & 100\% & 0.143 & 0.821 & 100\% & -0.224 & 0.750 & 100\% & -0.223 & 0.821 & 100\% \cr
 \midrule
 
 \begin{tabular}[c]{@{}c@{}}16b-1-1-0-0\\ -dc-2-2-0\end{tabular} & 0.382 & 0.900 & 100\% & 0.534 & 0.821 & 100\% & 0.475 & 0.722 & 100\% & -0.161 & 0.722 & 100\% & -0.052 & 0.788 & 100\% \cr
 \midrule
 
 \begin{tabular}[c]{@{}c@{}}1b-4-2-0-0\\ -dc-2-2-0\end{tabular} & 0.618 & 1.000 & 100\% & 0.196 & 0.742 & 100\% & 0.216 & 0.821 & 100\% & -0.149 & 0.821 & 100\% & -0.242 & 0.821 & 100\% \cr
 \midrule
 \midrule
 \begin{tabular}[c]{@{}c@{}}Overall similarity \\ of Approach $\triangle$ \end{tabular} & - & - & - & - & - & - & 0.206 & 0.674 & -  & -0.185 & 0.393 & - & -0.132 & 0.450 & -  \cr
 \midrule
  
 \begin{tabular}[c]{@{}c@{}}Overall similarity \\ of \Name \end{tabular} & 0.453 & 0.870 & 100\% & 0.296 & 0.855 & 100\% & 0.206 & 0.807 & 100\%  & -0.185 & 0.722 & 90\% & -0.132 & 0.734 & 94\%  \cr

   \bottomrule
    \end{tabular}
    \end{threeparttable}
}
 \vspace{-0.1in}
  \label{table:opencresult}
\end{table*}
}

\textbf{Semantic Equivalence.}
%%Although \Name could deobfuscates the BCF approach to binary level, we opt to use I/O approach to automatically evaluate our deobfuscation results are semantic equivalent to the original ones.
As shown in Table~\ref{table:opencresult} (cf. Column ``SE''),
all deobfuscation results are equivalent to the original ones, for the two levels of BCF obfuscation. 
We further manually checked the deobfuscation results of the 16 functions shown in Table~\ref{table:opencresult} by analyzing the instructions in each block of the CFGs, and found that their semantics are indeed equivalent to the original ones. 

% 正如表格2中列SE所示，针对BCF的所有反混淆结果都是与原始语义完全等价的。
% 




% By analyzing the obfuscated programs, we can see that when using BCF of the same intensity, if the structure of a program is more complicated, the obfuscated function is much closer to the unobfuscated situation. When the structure of the function is relatively simple, the impact of introducing bogus branches will become relatively large.
% We use selectionsort as an example to illustrate this situation.

% \haoyu{this sentence is not fully correct. should rewrite or delete}

% The obfuscation at default level of BCF shows an average similarity score of 0.452978, with a total number of 94 functions. The average recovered similarity of this benchmark is 0.870141. 

% In order to better show the effect of our method, we have analyzed the case where the obfus. probability is 50\%. At this level of obfuscation, the gap between results of the various functions becomes smaller but still exists. We use selectionsort as an example to illustrate this situation.




% As Fig.\ref{select-bcf} illustrates, the unobfuscated selectionsort function is an algorithm with a relatively complex structure. While obfuscating by default BCF, the obfuscator only introduced a dead branch which leads to a self-looping block. When the obfuscation strength is increased, it can be seen that the lower half of the obfuscation program is significantly different from the unobfuscated one. The reason for this phenomenon is BCF is a obfuscating approach with probability. 
% If the obfuscator wants to make confusion on the lower half, it needs to modify more basic blocks to ensure the operation of the original function.

% The difference between the recovery result and the unobfuscated function mainly caused by block splitting. The insertion of opaque predicates separates the original block, which leads to the difference in control flow. Since there are some other assignment operations in the Predicate Block, we have not merged these two blocks. In actual analysis, such differences do not lead to misjudgment of program understanding. For other functions, the difference between the recovery result and the original function is also mainly caused by such a reason.

% Also in Table.~\ref{table:opencresult}, there are a few functions, such as \textit{``lcm''} and \textit{``decimaltobinary''}, show a decline in the obfuscation effect when the obfuscation strength is raised. We believe that this inverse growth is due to the BCF-specified pattern of obfuscation with probability too. For a function, higher obfuscating ratio from the obfuscator does not necessarily resulting into more bogus branches and dead blocks added. 


% \begin{table*}[t]
% \renewcommand\arraystretch{1.5}
% \centering
% \label{table:opencbenchmark}
% \caption{CFG Similarity on C/C++ Obfuscation Benchmark}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{9B9B9B} 
% Category & Name & BCF & BCF\_re & BCF\_50\% & BCF\_50\%\_re & CFF & CFF\_re & CFF-3 & CFF-3\_re & ALL & ALL\_re \\ \hline
%  
%   & selectionsort & 0.903614 & 0.937500 & 0.398374 & 0.937500 & 0.151316 & 0.910256 & -0.160305 & 0.875000 & -0.128099 & 0.747126 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ Sort} & bubblesort & 0.708861 & 0.852459 & 0.469388 & 0.969697 & 0.200000 & 0.818182 & -0.160377 & 0.726027 & -0.230469 & 0.820896 \\ \hline
%  
%   & binarysearch & 0.758621 & 0.897436 & 0.371901 & 0.923077 & 0.136986 & 0.868421 & -0.191571 & 0.868421 & 0.023077 & 0.816327 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ Search} & binarysearchrec & 0.597222 & 0.750000 & 0.326087 & 0.750000 & 0.318182 & 0.843137 & -0.130178 & 0.816327 & 0.023077 & 0.816327 \\ \hline
%  
%   & gcd & 0.660377 & 0.871795 & 0.388060 & 0.871795 & 0.075269 & 0.775510 & -0.210526 & 0.775510 & -0.293578 & 0.775510 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ Math} & lcm & 0.151515 & 0.911765 & 0.365385 & 1.000000 & 0.171875 & 0.857143 & -0.218045 & 0.911765 & -0.218045 & 0.911765 \\ \hline
%  
%   & concatstrings & 0.213333 & 0.769231 & 0.132530 & 0.795455 & 0.213333 & 0.777778 & -0.260606 & 0.871795 & -0.124031 & 0.871795 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ String} & reverse & 0.280000 & 1.000000 & 0.369565 & 0.900000 & 0.291667 & 0.925926 & -0.252174 & 0.827586 & -0.113636 & 0.827586 \\ \hline
%  
%   & romannumerals & 0.234043 & 0.796813 & 0.321168 & 0.816092 & 0.164241 & 0.796813 & -0.249533 & 0.868996 & -0.340249 & 0.806867 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ Num2String} & decimaltobinary & 0.184466 & 0.905660 & 0.252632 & 0.782609 & 0.310345 & 0.854167 & -0.174157 & 0.854167 & 0.015748 & 0.854167 \\ \hline
%  
%   & bkdrhash & 0.175439 & 0.827586 & 0.155172 & 0.822222 & 0.294118 & 0.925926 & -0.165049 & 0.827586 & -0.069767 & 0.925926 \\ \cline{2-12} 
%  
% \multirow{-2}{*}{ Hash functions} & djbhash & 0.377778 & 0.827586 & 0.409091 & 0.812500 & 0.264151 & 0.925926 & -0.173077 & 0.925926 & -0.198198 & 0.741935 \\ \hline
%  
% \begin{tabular}[c]{@{}c@{}}Number of IF\\ -statements\end{tabular} & \begin{tabular}[c]{@{}c@{}}1b-1-2-2-1-\\ gt127-0-0-0\end{tabular} & 0.617647 & 1.000000 & -0.028571 & 1.000000 & 0.304348 & 1.000000 & -0.134831 & 1.000000 & -0.126437 & 1.000000 \\ \hline
%  
% \begin{tabular}[c]{@{}c@{}}Number of input dependent\\  IF-statements\end{tabular} & \begin{tabular}[c]{@{}c@{}}1b-1-2-1-1-gtsum\\ 127\_dep-1-0-1\end{tabular} & 0.617647 & 0.892857 & 0.083333 & 0.736842 & 0.142857 & 0.821429 & -0.223881 & 0.750000 & -0.223301 & 0.814815 \\ \hline
%  
% Number of loops & \begin{tabular}[c]{@{}c@{}}16b-1-1-0-0\\ -dc-2-2-0\end{tabular} & 0.382353 & 0.900000 & 0.534483 & 0.820513 & 0.474576 & 0.722222 & -0.160584 & 0.722222 & -0.052083 & 0.787879 \\ \hline
%  
% \begin{tabular}[c]{@{}c@{}}Number of input \\ dependent loops\end{tabular} & \begin{tabular}[c]{@{}c@{}}1b-4-2-0-0\\ -dc-2-2-0\end{tabular} & 0.617647 & 1.000000 & 0.196078 & 0.741935 & 0.215686 & 0.821429 & -0.149425 & 0.821429 & -0.242991 & 0.821429 \\ \hline
%  
% Average &  & 0.452978 & 0.870141 &  &  & 0.205562 & 0.806897 &  &  &  &  \\ \hline
% \end{tabular}}
% \end{table*}
% \end{landscape}

% For BCF, we restored deobfuscating work to binary on the open source benchmark. And recovered binaries are all manually verified according to the constraints in source codes. The execution results of all recovery files are correct. But in order to better show the results, we use the CFG similarity for evaluation.

% In Table.\ref{opencoure}, column ``BCF'' and ``BCF\_50\%'' indicate situations of default and bcf\_prob=50\% respectively. Column's name add ``\_re'' means the deobf. result of that obfus. 
% As the data shows, the obfuscation at default level of BCF shows a average similarity score of 0.452978, with a total number of 94 functions. The average recovered similarity of this benchmark is 0.870141. The data shows that the obfuscation under this intensity appears to be polarized. After analyzing these programs, we found that once the structure of a program is more complicated, the obfuscated function is more closer to the unobfuscated situation. When the structure of the function is relatively simple, the impact of introducing bogus branches will become relatively large. 

% \begin{figure}[htbp]
% \centering
% \begin{minipage}[]{0.2\columnwidth}
% \includegraphics[width=0.5\columnwidth]{pictures/select-origin.png}
% \end{minipage}%
% \begin{minipage}[]{0.2\columnwidth}
% \includegraphics[width=0.5\columnwidth]{pictures/select-30.png}
% \end{minipage}
% \begin{minipage}[]{0.2\columnwidth}
% \includegraphics[width=0.5\columnwidth]{pictures/select-50.png}
% \end{minipage}
% \begin{minipage}[]{0.2\columnwidth}
% \includegraphics[width=0.5\columnwidth]{pictures/select-re.png}
% \end{minipage}
% \caption{selectionsort}
% \label{select-bcf}
% \end{figure}

% \begin{figure}[htbp]
% \centering
% \includegraphics[width=0.8\columnwidth]{evaluation_pic/BCF-selectionsort.png}
% \caption{selectionsort}
% \label{select-bcf}
% \end{figure}

\subsubsection{Control Flow Flattening}

% Then we moved our line of sight to the deobfuscation of Control Flow Flatten. 
% \haoyu{rewrite this paragraph with the following texts, just describe what does it mean.}

\mbox{} \\ 
CFF offers an additional obfuscating option \texttt{split\_num}, which means to split the original basic block a specified number of times, to increase the complexity of obfuscated control flow.
In the evaluation, we have applied two different obfuscation levels: the default CFF obfuscation\footnote{O-LLVM itself does not split the basic block. However, due to optimizations during ARM compilation, basic block splitting still exists to some extent.}, and an enhanced obfuscation level with the basic block splitting option on \texttt{split\_num=3}.
% \haoyu{rewrite}. 
% The results of these two situation are shown in column 'CFF' and 'CFF-3'. And the column name add '\_re' is the deobf. similarity score of that situation.

% , as a result, the deobfuscationg work for this pass is also the focus of our evaluation. 


% We started from deobfuscation work on open source C benchmark with control flow flatten at default setting. 

% \haoyu{Overall results here.} 


\textbf{Result.} Table \ref{table:opencresult} shows the results. Column \textit{``CFF''} and Column \textit{``CFF\_re''} shows the results on default obfuscation of CFF, and Column \textit{``CFF-3''} and Column \textit{``CFF-3\_re''} shows the results of enhanced obfuscation, respectively. 
Obviously, with CFF obfuscation, the obfuscated code achieved significant differences compared to original ones considering the CFG similarity. 
At the default obfuscation level, the average CFG similarity score is only 0.206 after obfuscation, while our deobfuscation results could achieve a similarity score of 0.807 on average. After activating basic block splitting, similarity scores between the obfuscated and original function are almost all negative correlation (-0.185 on average), which indicates that the obfuscated CFG is completely different from the original one. The listed deobfuscation result of the enhanced CFF ranges from 0.72 to 1. The average value on all 90 functions(4 failures with O-LLVM compiling) is 0.722.


% \haoyu{One paragraph here to clearly describe the example! Merge all the following TEXTS!}

% While CFF obfuscating approach being used, the function produces significant differences compare to the unobfuscated one. By default obfuscate setting, the average score of CFG similarity is 0.205562, and some of them are even lower than 0.1. And our deobfuscation result got an average score of 0.806897 on a total number of 94 functions. After activating basic block split mode, similarity scores between the obfus. and unobfus. function are almost all negative correlation, which indicates that the obfuscated CFG is completely different from the unobfuscated one. 

% \begin{figure*}[htbp]
% \centering
% \begin{minipage}[t]{0.15\linewidth}
% \includegraphics[width=\linewidth]{evaluation_pic/16-origin.png}
% \label{fig:16-origin}
% \caption{Unobf.}
% \end{minipage}%
% % \begin{minipage}[t]{0.2\linewidth}
% % \includegraphics[width=\linewidth]{pictures/16-1.png}
% % \label{fig:side:b}
% % \end{minipage}
% \begin{minipage}[t]{0.5\linewidth}
% \includegraphics[width=\linewidth]{pictures/16-3.png}
% \label{fig:16-3}
% \caption{Obf.}
% \end{minipage}
% \begin{minipage}[t]{0.25\linewidth}
% \includegraphics[width=\linewidth]{evaluation_pic/16-re.png}
% \caption{Deobf.}
% \label{fig:16-re}
% \end{minipage}
% \end{figure*}




% As the data shows, except a few functions, our system achieves close results on both cases of a same function. 
% We first use program 16b-1-1-0-0-dc-2-2-0 as example to illustrate the reason why gaps occur between the Deobf. and Obf. function.


\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{evaluation_pic/16.pdf}
\vspace{-0.15in}
\caption{A Deobfuscation Example of CFF.}
\label{fig:16}
\vspace{-0.1in}
\end{figure}


\textbf{Case Study.} Experimental results suggest that our approach could achieve promising results on most cases. However, for several cases, the CFG similarity of deobfuscated code with the original binary is roughly 0.7. By further analyzing these cases, we found that the main reason is the redistribution of semantics in the original basic blocks. We use the program 16b-1-1-0-0-dc-2-2-0 as an example to illustrate this situation.
As shown in Fig. \ref{fig:16}. This is a function that calculates twice the sum of the ASCII codes of the input string. 
% To clearly show our deobfuscated result, we display the key instructions of each basic block in the CFG. 
The program got a recover result of 0.722 in both default and enhanced obfuscation. 
% The recovered CFG is shown in Fig. \ref{fig:16}. 
Block A in the original CFG (Fig. \ref{fig:16} (a)) is a transition block, and we assume that its parent and child node are directly connected. Also, the two self-loop basic blocks in the original CFG become the loop between two blocks in the recovered result. The key operation `ADD' of the two self-loop structures in the original function are now implemented in the split-out blocks B and C, as shown in Fig. \ref{fig:16} (c). Thus operations on edges D and E can be merged to another branch of its starting node.
This example suggests that CFF may separate constraints and operations during obfuscation, which will lead to re-matching of nodes and edges in the recovered result. 
However, this scenario will not affect the analyzing results, but instead simplifying the analysis process. 

\textbf{Semantic Equivalence.} Here we also use the \texttt{I/O} approach to check whether our deobfuscation results are semantic equivalent to the original ones.
As shown in Table~\ref{table:opencresult} (cf. Column \textit{``SE''}), for the default CFF obfuscation, our deobfuscation results are totally identical with the original semantics.
However, for the enhanced CFF obfuscation, we found some cases shared different outputs with original ones, thus the overall semantic equivalent evaluation result is 90\%. 
By analyzing these exceptional cases, we found that the main reason is introduced by function splitting (cf. Figure~\ref{fig:uninit}), as we skipped the \texttt{BL and BLX} instructions when we perform the semantic equivalence evaluation.
For such exceptional cases, we manually compared the deobfuscated programs and the original ones, and found that their semantics should be identical if we consider the \texttt{BL and BLX} instructions (superimposing the recovered functions), which we will elaborate in both following subsection and Section~\ref{sec:discussion}
%%the \texttt{I/O} approach we use skipped the \texttt{BL} instruction. We will further discuss it in Section 8.

%%deobfuscation results for CFF on C/C++ obfuscation benchmark in both two cases(default and enhanced) are completely equivalent to the original semantics. The \texttt{I/O} percentage of semantic equivalent samples in total is 100\% in the default CFF case. The value decreased to 89\% in the enhanced CFF case.
%%We also manually analyzed the deobfuscation results of the 16 functions shown in Table~\ref{table:opencresult}, and proved that their semantics are completely equivalent to the original semantics. 


% Now the difference between the result of the recovered and the unobfuscated function lies in edges D and E. But there are almost no operations on edges D and E. In the recovered control flow, due to the splitting of the instructions, the work done by the two branches in the unobfuscated function can be completed by one path. The control flow in recovered CFG can go through the first 3 blocks and 'do nothing'.


% Additionally, there are some functions that differs in the recovery results under different obfuscation strengths. Among programs we analyzed, many unobfuscated functions that originally had a multi-branch structure may lose some edges in the recovered CFG. The reason for this is that CFF sometimes separates constraints and operations during obfuscation, which leads to changes in nodes and edges of recovered control flow. It is natural to affect the similarity scores. In the actual analysis process, such situations will not affect the analysis, but instead simplify the analysis process. 
% \haoyu{TODO}
% todo

\subsubsection{Full Obfuscation (All 3 Techniques)}
\mbox{} \\ 
The aforementioned results suggest that \Name can recover the obfuscated samples accurately for each pass of O-LLVM. We further evaluate it if three obfuscation techniques are used at the same time.


% After completing the separate analysis of the two obfuscation methods, we implement our deobfuscation system on the mixture situation of O-LLVM's three passes. 

\textbf{Result.} The result is shown in the last three Columns in Table \ref{table:opencresult}. Obviously, the combined techniques introduce strong obfuscation impacts, with negative CFG similarity scores for most cases. The average CFG similarity score after obfuscation is -0.132 on average. However, \Name could achieve good results compared with single pass evaluation, with an average CFG similarity score of 0.734 after deobfuscation. For example, the \textit{romannumberals} function, which converts decimal numbers to Roman characters, has more than 500 basic blocks after hybrid obfuscation of O-LLVM. The CFG similarity score of the obfuscated function is -0.340, which is the lowest. The deobfuscating result on \textit{romannumberals} is 0.807, showing that \Name is resilient to complicated code obfuscation.
% , even though we have no prior knowledge about which techniques are used.

\textbf{Semantic Equivalence.} 
We further perform semantic equivalence evaluation.
As shown in the last column of Table~\ref{table:opencresult}, besides several exceptional cases (e.g., bkdrhash), we could get identical outputs for most cases, and thus the final average result is 94\%. Note that we further manually analyzed the extreme cases, and found the leading reason is the same with the cases we identified in CFF deobfuscation, i.e., function splitting (cf. Section~\ref{sec:discussion}).

%%The \texttt{I/O} approach is also used here to automatically prove deobfuscation results are semantic equivalent to the original ones. As Column \textit{``SE''} in Table~\ref{table:opencresult} shows, all listed 16 deobfuscation results for full obfuscation on C/C++ obfuscation benchmark are completely equivalent to the original semantics. The \texttt{I/O} percentage of semantic equivalent samples in total is 94\%. We also manually analyzed the deobfuscation results of the 16 functions shown in Table~\ref{table:opencresult}, and proved that their semantics are completely equivalent to the original semantics. 



\subsubsection{Comparing with Existing Studies.}
\mbox{} \\ 
%In previous studies, Francis Gabriel~\cite{gabriel2014deobfuscation} attempted to recover O-LLVM obfuscated code on the X86 platform. His work is based on the Miasm~\cite{miasm} framework to reverse the obfuscated function only to a CFG in all three kind of obfuscation approaches in O-LLVM. However, as we illustrated in Section \ref{sec:background}, it did not tackle multiple challenges introduced by ARM and Android. 
In previous studies, Francis Gabriel~\cite{gabriel2014deobfuscation} attempted to recover O-LLVM obfuscated code on the X86 platform based on the Miasm~\cite{miasm} framework. Specifically, his work only aimed to recover corresponding CFGs of functions protected by one of the three obfuscating techniques in O-LLVM. However, as we illustrated in Section \ref{sec:background}, it did not tackle multiple challenges introduced by ARM and Android. 

In this subsection, we would like to compare his work (we use the symbol $\triangle$ to represent it) with ours. Because the Approach $\triangle$ could not be used to deobfuscate Android native functions directly, we make the compromise to remove the context inheritance algorithm and control flow reconstructing rules in \Name and assume that Approach $\triangle$ could achieve the alike deobfuscation result with the degraded \Name. Obviously it is unfair to our approach considering the adoption of numerous improvements and innovations beside these two dominating ideas. However, if \Name could produce better results than Approach $\triangle$ in this scenario, the deobfuscating ability of \Name will be convincing. 
% not basic, it's ACE idea, lol

As shown in Table \ref{table:opencresult}, not surprisingly, the average similarities of the obfuscated functions in these three cases (CFF, CFF-3 and ALL) are exactly the same. However, the average deobfuscated CFG similarity of Approach $\triangle$ in the CFF situation is 0.674. Even worse, the similarity values decline dramatically to 0.393 and 0.450, CFF-3 and ALL respectively. With regard to those relatively large or basic-block-split functions, our further manual investigation demonstrates that the recovered result of Approach $\triangle$ is fragmented, and the corresponding caller-callee relationships between many basic blocks are lost, i.e., there does not exist any recovered path to reach the Return block. Due to its essence of unreliable results, we do not use the \texttt{I/O} approach to prove the correctness of Approach $\triangle$.
As such, we have demonstrated that \Name could achieve more accurate and convincing deobfuscation results.


% The deobfuscating result on \textit{romannumberals} is 0.807, which suggests that our approach is resilient to complicated obfuscation.




% basic block splitting and instruction optimization, which pose a great challenge for both x86 and ARM platforms. Besides, they did not provide an effective method to identify the obfuscation techniques used in a binary. Finally, context inheritance and sub-function calls are not considered in their work, which is more likely to fail when analyzing large programs.



% 's column 'ALL' and 'ALL\_re'. As data shows, when the three passes are activated at the same time, the Obfus. CFG similarity are almost all negative. It indicates that the Obfus. CFG is totally different from the Unobfus. one. It becomes very complicated.
% But on this situation, our deobfuscating approach produces a very similar control flow graph to the Unobf. one on most functions, with the Deobf. similarity scores around 0.8. It is noticeable that \textit{romannumberals} is a function with more than 500 basic blocks after obfuscation. Our deobfuscating system still achieved good result on such a large program.
% The exception is the romannumberals function, which convert decimal numbers to Roman characters. The obfuscator generates a CFG with more than 400 basic blocks in this obfuscation mode. Due to the limitation of time, we cannot find out the reason. But this function in 'CFF-3' mode is much bigger than 'ALL' situation(though with lower CFG similarity score). DiAna also got a good recover result on 'CFF-3' situation.
% There are some functions having more than hundreds of basic blocks, such as gcd and romannumberals, 

\begin{table}[t]
\centering
\caption{Deobfuscation result on open-source Android apps.}
%%\vspace{-1ex}
\resizebox{1\linewidth}{!}{

  \begin{threeparttable}


    \begin{tabular}{c|c|ccc|ccc}
    \toprule
    APK Name & Function Name & CFF & CFF\_re & SE & BCF & BCF\_re & SE 
    \cr
    \midrule
 & rdft & 0.199 & 0.919 & 100\% & 0.166 & 0.702  & 100\%\cr 
 & newFFT & 0.174 & 0.792 & 100\% & 0.704 & 0.792  & 100\%\cr 
 & makect & 0.325 & 0.913 & 100\% & 0.244 & 0.786  & 100\%\cr 
 \multirow{-4}{*}{Practice Hub} & Total  10 & 0.365 & 0.843 & 100\% & 0.446 & 0.795  & 100\%\cr
 \midrule
  
  & \begin{tabular}[c]{@{}c@{}}free\end{tabular} & 0.228 & 0.889  & 100\%& 0.338 & 0.752  & 100\%\cr
 
 & \begin{tabular}[c]{@{}c@{}}seekToFrame\end{tabular} & 0.017 & 0.725 & 100\% & 0.537 & 0.795  & 100\%\cr
 
 & \begin{tabular}[c]{@{}c@{}}seekToTime\end{tabular} & -0.004 & 0.698  & 100\%& 0.607 & 0.871  & 100\%\cr
 

\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Overchan\end{tabular}}  & Total 17 & 0.138 & 0.745 & 94\% & 0.339 & 0.761 & 100\% \cr
 \midrule
%  fillPixelsInRowNative
% getAsciiValuesBWNative
%getAsciiValuesWithColorNative
  & \begin{tabular}[c]{@{}c@{}}InRowNative\end{tabular} & 0.389 & 0.717 & 100\% & 0.457 & 0.654 & 100\% \cr
 & \begin{tabular}[c]{@{}c@{}}BWNative\end{tabular} & 0.417 & 0.714 & 100\% & 0.683 & 0.892 & 100\% \cr
 & \begin{tabular}[c]{@{}c@{}}ColorNative\end{tabular} & 0.009 & 0.712 & 100\% & 0.486 & 0.712 & 100\% \cr 
\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}AsciiCam\end{tabular}} & Total  3 & 0.266 & 0.714 & 100\% & 0.542 & 0.753 & 100\% \cr
 \midrule
  
 & anagrams\_init & 0.133 & 0.802 & 100\% & 0.143 & 0.911 & 100\%\cr  
  
 & \begin{tabular}[c]{@{}c@{}}Anagrams\_uninit\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.791
(0.077)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.333
(0.875)\end{tabular}  & 27(100)\% & \begin{tabular}[c]{@{}c@{}}0.800
(0.122)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.160
(0.810)\end{tabular}  & 21(100)\%\cr 
  
  & anagram & 0.174 & 0.830 & 100\% & 0.058 & 0.784 & 100\%\cr 
  

\multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Agram\end{tabular}}  & Total 24 & 0.198 & 0.761 & 100\% & 0.511 & 0.777 & 100\% \cr 
 \midrule
 & createWnnWork & 0.067 & 0.747 & 100\% & 0.306 & 0.848  & 100\%\cr 
 & freeWnnWork & 0.149 & 0.875 & 100\% & 0.316 & 0.737  & 100\%\cr 
\multirow{-3}{*}{NicoWnnG} & Total 2 & 0.108 & 0.811  & 100\%& 0.311 & 0.792  & 100\%\cr 
   \bottomrule
    \end{tabular}
    \end{threeparttable}
    
}
\vspace{-4ex}
\label{table:mobileresult}
\end{table}

\subsection{\textbf{Evaluation on Open-Source Android Apps}}



% \begin{table*}[!htbp]
% \label{table:mobileresult}
% \caption{Deobfuscation Result of Open Source Android Apps}
% \renewcommand\arraystretch{1.5}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% APK Name & Function Name & CFF & CFF\_re & BCF & BCF\_re \\ \hline
%  & rdft & 0.198718 & 0.918605 & 0.165714 & 0.701923 \\ \cline{2-6} 
%  & newFFT & 0.173913 & 0.791667 & 0.703704 & 0.791667 \\ \cline{2-6} 
%  & makect & 0.325000 & 0.913043 & 0.244444 & 0.785714 \\ \cline{2-6} 
% \multirow{-4}{*}{Practice Hub} & Total  10 & 0.3647263 & 0.8427591 & 0.445744666667 & 0.795405222222 \\ \hline
%  & \begin{tabular}[c]{@{}c@{}}Java\_nya\_miku\_wishmaster\_\\ lib\_gifdrawable\_GifDrawable\_free\end{tabular} & 0.227848 & 0.888889 & 0.337931 & 0.752475 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_nya\_miku\_wishmaster\_lib\_\\ gifdrawable\_GifDrawable\_seekToFrame\end{tabular} & 0.017442 & 0.725000 & 0.536842 & 0.794872 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_nya\_miku\_wishmaster\_lib\_\\ gifdrawable\_GifDrawable\_seekToTime\end{tabular} & -0.003704 & 0.697674 & 0.607143 & 0.870690 \\ \cline{2-6} 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Overchan\end{tabular}} & Total 17 & 0.138025619048 & 0.745454809524 & 0.339112705882 & 0.761267 \\ \hline
%  & \begin{tabular}[c]{@{}c@{}}Java\_com\_dozingcatsoftware\_asciicam\\ \_AsciiRenderer\_fillPixelsInRowNative\end{tabular} & 0.388889 & 0.716981 & 0.456522 & 0.653846 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_com\_dozingcatsoftware\_asciicam\_\\ AsciiConverter\_getAsciiValuesBWNative\end{tabular} & 0.417391 & 0.714286 & 0.683168 & 0.892857 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_com\_dozingcatsoftware\_asciicam\_\\ AsciiConverter\_getAsciiValuesWithColorNative\end{tabular} & 0.008734 & 0.711712 & 0.485507 & 0.711712 \\ \cline{2-6} 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}AsciiCam\end{tabular}} & Total  3 & 0.265848666667 & 0.714326333333333 & 0.541732333333333 & 0.752805 \\ \hline
%  & anagrams\_init & 0.132979 & 0.802083 & 0.142857 & 0.911111 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_us\_achromaticmetaphor\_\\
% agram\_Anagrams\_uninit\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.790698\\
% (0.076923)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.333333\\
% (0.875000)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.800000\\
% (0.121951)\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.160000\\
% (0.809524)\end{tabular} \\ \cline{2-6} 
%  & anagram & 0.174419 & 0.829787 & 0.058252 & 0.784314 \\ \cline{2-6} 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}Agram\end{tabular}} & Total 24 & 0.198205 & 0.761010 & 0.511479 & 0.777419 \\ \hline
%  & \begin{tabular}[c]{@{}c@{}}Java\_net\_gorry\_android\_input\_nicownng\_\\ OpenWnnDictionaryImplJni\_createWnnWork\end{tabular} & 0.066667 & 0.746667 & 0.306306 & 0.848485 \\ \cline{2-6} 
%  & \begin{tabular}[c]{@{}c@{}}Java\_net\_gorry\_android\_input\_nicownng\_\\ OpenWnnDictionaryImplJni\_freeWnnWork\end{tabular} & 0.148936 & 0.875000 & 0.315789 & 0.736842 \\ \cline{2-6} 
% \multirow{-3}{*}{\begin{tabular}[c]{@{}c@{}}NicoWnnG\end{tabular}} & Total 2 & 0.1078015 & 0.8108335 & 0.3110475 & 0.7926635 \\ \hline
% \end{tabular}}
% \end{table*}

The five open source Android apps used in our evaluation are: (1) Practice Hub (com.proch.practicehub.src), a tool for musicians; (2) Overchan (bus.chio.wishmaster), an app for browsing different kinds of imageboards; (3) AsciiCam (com.dozing catsoftware.asciicam), a photography app generates ASCII images in real time, with more than 100K downloads in Google Play; (4) Agram (us.achromatic metaphor.agram), a tool to list single-word and multi-word anagrams in English; (5) NicoWnnG (net.gorry.android.input.nicownng), a keyboard IME with more than 50K downloads in Google Play.

\textbf{Result.} For each open-source app, we first extract its native source code. Then we use O-LLVM to perform obfuscation when building $*.so$ according to Application.mk and Android.mk in the original Android projects.
% for obfuscation compilation of these native code according to the original Application.mk and Android.mk in their project folders\haoyu{rewrite}. 
In the deofuscation process, we filtered the functions that contain only one basic block. At last, we analyzed 56 functions in total. 
% Because the previous result did not show a big difference under different strength of obfuscation, we analyzed all functions that obfuscated by default CFF and BCF separately.

% using our deobfuscation system and then used O-LLVM for obfuscation compilation of these native code according to the original Application.mk and Android.mk in their project folders.

Table \ref{table:mobileresult} shows the overall deobfuscation results. 
For binaries obfuscated with BCF (with average CFG similarity score ranging from 0.311 to 0.542), our approach could achieve a CFG similarity score in the range from 0.753 to 0.795 on average after deobfuscation. For binaries obfuscated with CFF (with average CFG similarity score ranging from 0.108 to 0.365), our approach could achieve a CFG similarity score around 0.75 on average after deobfuscation. Although the overall result is acceptable, for a few cases, our approach did not achieve good results as other cases. We further manually analyzed these cases.


{\begin{figure}[t]
\includegraphics[width=\columnwidth]{evaluation_pic/func-split.pdf}
%%\vspace{-0.2in}
\caption{Another deobfuscation case (Anagrams\_uninit).}
\label{fig:uninit}
%%\vspace{-0.1in}
\end{figure}}




\begin{figure*}[t]
\includegraphics[width=\linewidth]{evaluation_pic/CVE.pdf}
\caption{CFG comparison of search\_goodnum: ((1) Deobfuscated Graph; (2) Unobfuscated Graph. \textit{Obfuscated Graph in Fig. ~\ref{fig:motivating}.})}
\label{fig:goodnum}
\vspace{-0.1in}
\end{figure*}



We found that the main reason leading to the CFG inconsistency is \emph{function splitting}. We use function \textit{``Anagrams\_uninit''} in \textit{``Agram''} to illustrate it. Sometimes an operation in the original $*.so$ can be implemented by one function, while in the obfuscated binary, part of this operation may be split out and used as a sub-function due to optimizations. As shown in Fig. \ref{fig:uninit} (2), the CFG of deobfuscated function only contains 4 basic blocks. In the first block, this recovered function calls \textit{``sub\_5F24''}, which is also obfuscated by O-LLVM. The deobfuscation of \textit{``sub\_5F24''} is shown in Fig. \ref{fig:uninit} (3). After superimposing these two recovered functions' CFG, it can be seen that the similarity between original and recovered CFG is very high. The deobfuscation results are 0.875 for CFF and 0.810 for BCF, compare to 0.333 and 0.16 respectively. This result suggests that function splitting could greatly affect the result. Thus, in our implementation, we take the function splitting into consideration, which is not carefully considered in previous studies~\cite{D-OLLVM2017,gabriel2014deobfuscation,yadegari2015generic}.


\textbf{Semantic Equivalence.} As shown in the Column \textit{``SE''} of Table~\ref{table:mobileresult}, except for app ``Overchan", all the recovered functions of the rest apps get 100\% identical outputs in our \texttt{I/O} approach. We further manually analyzed such cases, and found that their semantics are completely equivalent to the original semantics, while this result is introduce by the limitation of our I/O approach (cf. Section~\ref{sec:discussion}).
%%We further manually analyzed the deobfuscation results of the 14 functions shown in Table~\ref{table:mobileresult}, and proved that their semantics are completely equivalent to the original semantics. 





% \haoyu{cite here}
% It can be seen that the negative impact on the result of this situation is very large. We do not think this is a drawback of our deobfuscation system, because function splitting can also only happen on unobfuscated functions, resulting in incomplete original information.\haoyu{To be modified} 


% \haoyu{totally unclear! rewrite this paragraph. Merge all the following texts into only one paragraph. } 


% We use figure to explain the meaning of function splitting. Sometimes an operation can be implemented by one function in the unobfuscated so library. But in the obfuscation function, part of operation may be splitted out and used as a sub-function. The sub-function will be obfuscated by O-LLVM too. Also the opposite situation may occur, that is, there are splits in the unobfuscated but not in the obfuscated function. As function 'Java\_us\_achromaticmetaphor\_agram\_Anagrams\_uninit' shown in Fig.\ref{fig:uninit}, the header of this function calls 'sub\_5F24', and 'sub\_5F24' is also obfuscated. After superimposing these two functions' recovered CFG, it can be seen that the similarity between unobfuscated and recovered CFG is still very high. 


% After completing the deobfuscation evaluation on the open source benchmark, we found that most deobfuscation results of our system are close on both the default and enhanced obfuscation. As a result, in the evaluation on Android project's so libraries, we choose the obfuscation with the default settings. Also, in the previous evaluation, the results of the experiment did not reflect that the mixed obfuscation of both BCF and CFF would have a great impact on the deobfuscation process and results. As a result, we did not analyze the 'ALL' obfuscated situation.

% For each so library, we have filtered out the function that contains only one basic block. For all the rest of functions, we analyzed them using our deobfuscating system, and results are shown in the table. It can be seen that the effect of deobfuscation has a slight decrease in the average value, compare to results on open source benchmark. We performed manual analysis on some bad results and found that these bad conditions are caused by function splitting.





% We show the score of CFG after superimposing in brackets.

% Due to the existence of the function split, the average score of our results is affected. The superimposing-CFG result of 'Java\_us\_achromaticmetaphor\_agram\_Anagrams\_uninit' is shown in table too. It can be seen that the negative impact on the result of this situation is very large. 


% 对于每个so库，我们晒去了只含有一个基本快的函数。对于其余的所有函数，都使用我们的反混淆系统进行了分析，得出的结果如表所示。可以看出，当单独使用BCF或者cff进行混淆的时候，平均结果略次于open上的
% 原因是因为，我们遇到了函数拆分的问题
% 图
% 这个问题我们认为不是我们的问题
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}

% \subsubsection{Bogus Control Flow}

% \subsubsection{Control Flow Flatten}

\begin{table}[t]
    \centering
  \fontsize{6.5}{8}\selectfont

  \begin{threeparttable}
  \caption{The deobfuscation result on the PoC implementation of towelroot.}
  \label{CVEtable}
%%  \vspace{-0.15in}
    \begin{tabular}{c|ccc|ccc}
    \toprule
    function name & CFF & CFF\_re & SE & ALL & ALL\_re & SE
    \cr
    \midrule
    accept\_socket & 0.302 & 0.797 & 100\% & -0.270 & 0.913 & 100\%  \cr 
 make\_socket &  0.346 &  0.667& 100\% &  -0.267 &  0.935& 100\%  \cr  
init\_exploit & 0.203 & 0.903& 100\% & -0.044 & 1.000& 100\% \cr 
 send\_magicmsg &  0.149 &  0.963& 100\% &  0.149 &  0.962& 100\%  \cr 
read\_pipe & 0.111 & 1.000 & 100\%& -0.265 & 1.000& 100\%  \cr  
 search\_goodnum &  0.193 &  0.939 & 100\%&  -0.245 &  0.900& 100\%  \cr 
make\_action & 0.367 & 1.000& 100\% & -0.157 & 0.850& 100\%  \cr  
 write\_kernel &  0.211 &  0.966& 100\% &  -0.210 &  0.703 & 100\% \cr 
wake\_actionthread & 0.216 & 0.927& 100\% & -0.220 & 0.912& 100\%  \cr 
 main &  0.194 &  1.000 & 100\% &  -0.253 &  0.652 & 100\% \cr 
write\_pipe & 0.111 & 1.000 & 100\% & -0.161 & 1.000 & 100\% \cr
   \bottomrule
    \end{tabular}
    \end{threeparttable}
    \vspace{-0.2in}
\end{table}


\subsection{Evaluation on Real-world Exploits}
% In this subsection, we would like to focus on Android Root Exploits (aka REs), a sort of binary tool which can be used to obtain the root privilege by exploiting privilege escalation vulnerabilities. 
% The use of REs was full of controversial~\cite{gasparis2017detecting}. On one side, as the key part of some legitimate products provided by root providers, REs have been used to serve normal customers for legal use (rooting, as well as jailbreak); on the other side, REs have already been embedded by malware in the wild to compromise the target Android devices. According to our observation, many embedded REs were obfuscated for various purposes, which became a big obstacle for security researchers.  

CVE-2014-3153~\cite{CVE2014} is a well-known generic vulnerabilities in the Linux kernel, i.e., the Fast User space muTEX (futex) subsystem, which is the basis of several mutual exclusion mechanisms. 
Its exploitation (e.g., towelroot~\cite{towelroot} and different variants) had been widely spread around world. The original towelroot was protected by O-LLVM, which took researchers a long time to understand the technical details by performing laborious reverse engineering. As shown in the motivating example (Fig.~\ref{fig:motivating}), it is quite difficult, if not impossible, for researchers (even experienced experts) to figure out the details from the obfuscated CFG directly. 


% The complexity comes from the essence of a race condition exploit with multiple threads, where the sequence of invoking system calls becomes the key to understand the subtle logic. 

\textbf{Result.} As of this writing, the source code of the original towelroot is still unavailable. Fortunately, some researchers have published their results, which can be regarded as the identical PoCs of the original one. We will then demonstrate the capability of our system based on one of them~\cite{git-cve}, and the results are summarized in Table \ref{CVEtable}. For simplicity, we focus on two key functions, i.e., ``search\_goodnum'' and ``send\_magicmsg'', to illustrate our work. 

% Looks like we do not need CFF results here.


The deobfuscation results of ``send\_magicmsg'' and ``search\_good-num'' in ``CFF'' situation are $0.963$ and $0.939$ respectively, which means that the deobfuscated CFGs are almost the same as the original ones. In ``ALL'' obfuscation situation, these two value are $0.962$ and $0.900$ respectively. Fig. ~\ref{fig:goodnum} shows the comparison between the two CFGs of ``search\_goodnum''. Compared to the obfuscated CFG shown in Fig.~\ref{fig:motivating}, it is obviously much easier to understand the logic of the exploitation, especially the system call sequences and key operands, from the deobfuscated CFG.

\textbf{Semantic Equivalence.} We also use the \texttt{I/O} approach to prove the deobfuscation results are semantic equivalent to the original function. As shown in Table \ref{CVEtable}, for all cases, all the outputs of deobfuscated functions are identical to the outputs of ones, considering the same 1,500 inputs.

% 几乎所有的反混淆函数与原始函数的输出是100%相同的，考虑在同样输入的情况下

% (the one with functionality description)
% The deobfuscation result of ``send\_magicmsg'' is $0.962$, 

% 考虑放一张图，介绍下CVE的功能啥的，然后介绍一个函数



% \begin{table}[]
% \renewcommand\arraystretch{1.5}
% \centering
% \begin{tabular}{|l|l|l|l|l|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% function name & CFF & CFF\_re & ALL & ALL\_re \\ \hline
% accept\_socket & 0.302326 & 0.791667 & -0.270492 & 0.913043 \\ \cline{2-4} 
%  make\_socket &  0.346154 &  0.666667 &  -0.267081 &  0.935484 \\ \cline{2-4} 
% init\_exploit & 0.203390 & 0.903226 & -0.044444 & 1.000000 \\ \cline{2-4} 
%  send\_magicmsg &  -0.021505 &  0.755556 &  -0.321586 &  0.500000 \\ \cline{2-4} 
% read\_pipe & 0.111111 & 1.000000 & -0.265060 & 1.000000 \\ \cline{2-4} 
%  search\_goodnum &  0.193333 &  0.939024 &  -0.245179 &  0.900000 \\ \cline{2-4} 
% make\_action & 0.3666673 & 1.000000 & -0.157143 & 0.850000 \\ \cline{2-4} 
%  write\_kernel &  0.211082 &  0.966184 &  -0.210462 &  0.702857 \\ \cline{2-4} 
% wake\_actionthread & 0.215686 & 0.927273 & -0.220339 & 0.912281 \\ \cline{2-4} 
%  main &  0.194444 &  1.000000 &  -0.252747 &  0.652174 \\ \cline{2-4} 
% write\_pipe & 0.111111 & 1.000000& -0.161290 & 1.000000 \\ \hline
% %  
% % Average & \sum(b2:b4) & 0 & 0 & 0 \\ \hline
% \end{tabular}
% \label{CVEtable}
% \caption{The deobfuscation result of towelroot's PoC}
% \end{table}


% Our experimental evaluation is divided into four parts. 
% In the first part, to evaluate the deobfuscating work of the instruction substitution, we selected five computationally intensive source code and built them into so library. 
% After applying our deobfuscating approach on them, we manually verifying the correctness of these five recovered functions. Then the Euclidean distances from the obfuscated function to the unobfuscated function, and from the deobfuscated function to the unobfuscated function are both calculated. 

% Secondly, we chose an open source benchmark~\cite{banescu2016code} and made deobfuscation of control flow flatten and bogus control flow on this dataset. Also, to illustrate the accuracy of our approach, we use both the default settings and enhanced settings on both obfuscation passes. Then the three-passes-mixed obfuscation is evaluated too. 

% This benchmark includes common basic algorithms, hash functions, and small programs(mainly containing combinations of IF, WHILE, and FOR structures)\footnote{We abandoned the source code automatically generated by RandomFuns in the tigress-generated-programs folder.}.
% Due to space limitations, and to show our experimental results more clearly, we have reclassified the source code in this benchmark. 

% As shown in Table 1, we divide the algorithms in basic algorithm folder into sorting algorithm(Sort), searching algorithm(Search), mathematical calculation(Math), string manipulation(String) and conversion between number and string(Num2String). For the source code in the small programs folder, we classify them according to their program structure. In addition, five source codes in the small program folder are too simple (i.e. the unobfuscated function has only one basic block), so we did not make analysis on them. 


% After completing the comprehensive deobfuscation analysis on the open source benchmark, we look into the deobfuscating accuracy of our approach on actual projects. We crawled some open source Android projects from F-Droid~\cite{} --- a website of the open source android project --- and filtered out projects that didn't use native code or use native code without source code. We finally use 5 projects to form a dataset and use O-LLVM obfuscator when building native source codes into .so files. We evaluate the accuracy of our deobfuscating approach on functions in these binaries.

% 第四部分，我们对于实际工作中遇到的使用ollvm进行混淆的漏洞利用函数，进行了反混淆验证
% We will look into the application of O-LLVM in practical engineering project in the last part of our experiment. 在研究过程中，我们发现CVE的那个so库是使用ollvm进行混淆的，blahblahblahblahblahblahblahblahblahblahblahblahblah blahblahblahblahblahblahblahblahblahblahblahblahblahblahblah
% 这部分老师想想怎么说比较好

% \subsubsection{Dataset}
% We performed experimental evaluation on three datasets.

% The first dataset is a open source dataset provided by Banescu~\cite{banescu2016code}, 

% We selected five projects using native code from F-Droid --- a website of the open source android project --- to form the second dataset. The principle of choice is XXXXXXX. 
% 并对CFF和BCF的反混淆工作进行了分析

% 第三个数据集，我们选择了实际使用了OLLVM进行混淆的一个CVE的漏洞利用so库，并对CFF的反混淆结果进行了分析
% third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third third 
% 2018-08-07
% \subsubsection{CFG Similarity Algorithm}

% From the reverse engineer’s perspective, control flow analysis is an important procedure. Also due to the difficulty of patching control flow flatten obfuscated native code at the assembly level, we use the similarity of control flow graph to illustrates the effectiveness of deobfuscation work. After researching related works, we adopted the algorithm of Hu~\cite{hu2009large} for computing the edit distance between two control flow graphs, which was proved to be the most accurate of four algorithms in Chan's work~\cite{chan2014method}.

% The basic idea of Hu's algorithm is to build a cost matrix that represents the costs of mapping the different nodes in two graphs \textbf{\(G_1\)} and \textbf{\(G_2\)}. Then the Hungarian algorithm [22] is used to find an optimal solution to the assignment problem in \(\mathcal{O}\)\((n^{3})\) time. After that, we use formula below to calculate the CFG similarity score:
% \begin{equation}
% sim(G_1,G_2) = 1-\frac{\sigma(G_1,G_2)}{|N_1|+|N_2|+|E_1|+|E_2|}\label{CFGSim}
% \end{equation}

% Here, \textbf{\(\sigma(G_1,G_2)\)} is the edit distance between \(G_1\) and \(G_2\), \(|N_i|\) is the number of nodes in \(G_i\), and \(|E_i|\) is the number of edges in \(G_i\). The score given by Pearson correlation~\cite{pearson1896mathematical} is in the range of [-1,1] with 1 indicating total positive correlation, 0 indicating no correlation, and -1 indicating negative correlation. In another word, the closer the score is to 1, the closer the structure of the two graphs are. A similarity score no more than 0 means that two graphs are completely dissimilar.

% \subsubsection{Instruction Substitution}

% % 图
% % 对于指令替换的混淆方式，我们将反混淆工作patch到binary层级。并对程序恢复的正确性进行了验证。另外，可从表中数据得知，当源代码中的计算操作很多时，混淆后的binary与未混淆的binary在指令层级有较大差距
% % 这里我不知道应该怎么说。。。
% % 2018-8-16 这里可以考虑过渡下

% \subsubsection{Bogus Control Flow and Control Flow Flatten}
% The deobfuscating work of BCF and CFF is done on same datasets, so we will discuss their recovery results together. For BCF, we restored deobfuscating work to binary on the open source benchmark~\cite{banescu2016code}. And recovered binaries are all manually verified according to the constraints in source codes. The execution results of all recovery files are correct. But in order to better show the results, we use the CFG similarity for evaluation.



% \paragraph{\textbf{Result on Open Source Benchmark}}
% The evaluation of deobfuscating bogus control flow is first performed on the open source benchmark. Here we consider two different situations, the obfuscation intensity of default setting and bcf\_prob=50\%, which indicates a basic block will be obfuscated with a probability of 50\%.

% \begin{table*}[htbp]
% \renewcommand\arraystretch{1.5}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{C0C0C0} 
% Category & Name & CFF & CFF\_re & BCF & BCF\_re & CFF-3 & CFF-3\_re & BCF\_50\% & BCF\_50\%\_re & ALL & ALL\_re \\ \hline
%  & selectionsort & 0.151316 & 0.910256 & 0.903614 & 0.937500 & -0.160305 & 0.875000 & 0.398374 & 0.937500 & -0.128099 & 0.747126 \\ \cline{2-12} 
% \multirow{-2}{*}{Sort} & bubblesort & 0.200000 & 0.818182 & 0.708861 & 0.852459 & -0.160377 & 0.696429 & 0.469388 & 0.969697 & -0.230469 & 0.820896 \\ \hline
%   &  binarysearch &  0.136986 &  0.868421 &  0.758621 &  0.897436 &  -0.191571 &  0.868421 &  0.371901 &   0.923077 &  0.023077 &  0.816327 \\ \cline{2-12} 
% \multirow{-2}{*}{ Search} &  binarysearchrec &  0.318182 &  0.843137 &  0.597222 &  0.750000 &  -0.130178 &  0.816327 &  0.326087 &  0.750000 &  0.023077 &  0.816327 \\ \hline
%  & gcd & 0.075269 & 0.775510 & 0.660377 & 0.871795 & -0.210526 & 0.775510 & 0.388060 & 0.871795 & -0.293578 & 0.483871 \\ \cline{2-12} 
% \multirow{-2}{*}{Math} & lcm & 0.171875 & 0.857143 & 0.151515 & 0.911765 & -0.218045 & 0.666667 & 0.365385 & 1.000000 & -0.218045 & 0.911765 \\ \hline
%   &  concatstrings &  0.213333 &  0.777778 &  0.213333 &  0.769231 &  -0.260606 &  0.871795 &   0.132530 &   0.795455 &  -0.124031 &  0.871795 \\ \cline{2-12} 
% \multirow{-2}{*}{ String} &  reverse &  0.291667 &  0.925926 &  0.280000 &  1.000000 &  -0.252174 &  0.827586 &  0.369565 &  0.900000 &  -0.113636 &  0.827586 \\ \hline
%  & romannumerals & 0.164241 & 0.796813 & 0.234043 & 0.796813 & -0.249533 & 0.868996 & 0.321168 & 0.816092 & -0.340249
%  & 0.428169 \\ \cline{2-12} 
% \multirow{-2}{*}{Num2String} & decimaltobinary & 0.310345 & 0.854167 & 0.184466 & 0.905660 & -0.174157 & 0.854167 & 0.252632 & 0.782609 & 0.015748 & 0.854167 \\ \hline
%   &  bkdrhash &  0.294118 &  0.925926 &  0.175439 &  0.827586 &  -0.165049 &  0.827586 &  0.155172 &  0.822222 & -0.069767 &  0.925926 \\ \cline{2-12} 
% \multirow{-2}{*}{ Hash functions} &  djbhash &  0.264151 &  0.925926 &  0.377778 &  0.827586 &  -0.173077 &  0.925926 &  0.409091 &  0.812500 &  -0.198198 &  0.741935 \\ \hline
% Number of IF-statements & \begin{tabular}[c]{@{}c@{}}1b-1-2-2-1-\\ gt127-0-0-0\end{tabular} & 0.304348 & 1.000000 & 0.617647 & 1.000000 & -0.134831 & 1.000000 & -0.028571 & 1.000000 & -0.126437 & 1.000000 \\ \hline
%  \begin{tabular}[c]{@{}c@{}}Number of input \\ dependent IF-statements\end{tabular} &  \begin{tabular}[c]{@{}c@{}}1b-1-2-1-1-\\ gtsum127\\ \_dep-1-0-1\end{tabular} &  0.142857 &  0.821429 &  0.617647 &  0.892857 &  -0.223881 &  0.750000 &  0.083333 &  0.736842 &  -0.223301 &  0.814815 \\ \hline
% Number of loops & \begin{tabular}[c]{@{}c@{}}16b-1-1-0-0\\ -dc-2-2-0\end{tabular} & 0.474576 & 0.722222 & 0.382353 & 0.900000 & -0.160584 & 0.722222 & 0.534483 & 0.820513 & -0.052083 & 0.787879 \\ \hline
%   \begin{tabular}[c]{@{}c@{}}Number of input \\ value dependent loops\end{tabular} &   \begin{tabular}[c]{@{}c@{}}1b-4-2-0-0\\ -dc-2-2-0\end{tabular} &  0.215686 &  0.821429 &  0.617647 &   1.000000 &  -0.149425 &  0.821429 &  0.196078 &  0.741935 &  -0.242991 &  0.821429 \\ \hline
% Average &  & 0.205562 & 0.806897 & 0.452978 & 0.870141 &  &  &  &  &  &  \\ \hline
% \end{tabular}}
% \label{opencbenchmark}
% \end{table*}



% The results of the similarity comparisons on open source benchmark are shown in Table I. Column labeled 'CFF' gives the control flow graph similarity of default control flow flatten obfuscated binaries with the original binaries; Column labeled 'BCF' gives the control flow graph similarity of default bogus control flow obfuscated binaries with the original binaries; 'CFF-3' means control flow flatten with flag -split\_num=3. 'BCF\_50\%' means bogus control flow with flag -bcf\_prob=50\%. Column labels add '\_re' are similarities of deobfuscated function with the original one. 'ALL' is the three-passes-mixed situation.

% Not surprisingly, the obfuscated programs are usually very different from the original code structurally. For these two obfuscation modes, the confusion logic of the bogus control flow is the pseudo-addition of the control flow, and the control flow flatten is the breaking and reconstruction of the entire control flow. So on almost all programs, the confusion of CFF is better than BCF. In the following-up analysis of results, we will firstly evaluate deobfuscation of these two approaches separately. Then the mixed up situation will be discussed.

% \textbf{\#1. Deobf. Results of BCF:}

% The obfuscation at default level of BCF shows a average similarity score of 0.452978, with a total number of 94 functions. The average recovered similarity of this benchmark is 0.870141. The data shows that the obfuscation under this intensity appears to be polarized. After analyzing these programs, we found that once the structure of a program is more complicated, the obfuscated function is more closer to the unobfuscated situation. When the structure of the function is relatively simple, the impact of introducing bogus branches will become relatively large. 
% In order to better show the effect of our method, we have analyzed the case where the prob is 50\%. At this level of obfuscation, the gap between results of the various functions becomes smaller but still exists. We use selectionsort as an example to illustrate this situation.

% \begin{figure*}[htbp]
% \begin{minipage}[]{0.2\linewidth}
% \includegraphics[width=0.5\linewidth]{pictures/select-origin.png}
% \label{fig:side:a}
% \end{minipage}%
% \begin{minipage}[]{0.2\linewidth}
% \includegraphics[width=0.5\linewidth]{pictures/select-30.png}
% \label{fig:side:b}
% \end{minipage}
% \begin{minipage}[]{0.2\linewidth}
% \includegraphics[width=0.5\linewidth]{pictures/select-50.png}
% \label{fig:side:b}
% \end{minipage}
% \begin{minipage}[]{0.2\linewidth}
% \includegraphics[width=0.5\linewidth]{pictures/select-re.png}
% \label{fig:side:b}
% \end{minipage}
% \caption{selectionsort}

% \end{figure*}
% % yuantu 
% % 30%
% % 50%
% % huifu
% % 这是一个程序结构相对复杂的函数，在30%的情况显示，混淆后的图与未混淆的图仅仅添加了一个分支（暂时），而50%的情况，函数的后半部分变得非常复杂


% \textbf{\#2. Example of Deobf. BCF:}

% As figure illustrate, the unobfuscated selectionsort function is an algorithm with a relatively complex structure. From the perspective of the control flow graph, its control flow before block A is relatively simple. Starting from basic block \textbf{A}, the nesting of the loop structure occurs, so that the confusion of the structure of the second half becomes difficult. If the obfuscator wants to make confusion in the second half, it needs to modify more basic blocks to ensure the operation of the original function. So under the default parameters, the effect of obfuscation is not strong. When the confusion strength is increased, we can see that the second half of the obfuscation program is significantly different from the original one. 

% For the recovery of these two kinds of confusion, the result is the same, which also proves the effectiveness of our deobfuscating system.
% The difference between the recovery result and the unobfuscated function mainly occurs near the block \textbf{A}. There is a loop between B and C in the unobfuscated graph. But in the recovered graph, the B node is separated by opaque predicates and becomes two nodes(C and D). Since there some other assignment operations in the opaque predicate block (D), we have not merged these two blocks. This is the only difference between Figure 1 and Figure 4, but in actual analysis, such differences do not lead to misjudgment of program understanding. For other functions, the difference between the recovery result and the original function is also mainly caused by such a reason.

% Also in this table, there are a few functions, such as lcm and decimaltobinary, show a decline in the obfuscation effect when the obfuscation strength is raised. We believe that this inverse growth is due to the BCF-specified pattern of obfuscation with probability. For a function, higher obfuscating ratio from the obfuscator does not necessarily resulting into more bogus branches and dead blocks added. 

% % On the obfuscation of the concatstring function in the case of reinforcement, we get the same CFG as the unobfuscated one, so we did not count the deobfuscating result of this case.
% % 为了更好地说明我们的方法在该pass上的效果，我们将对进行50%和*100%（考虑周六把100%的做了）的混淆，结果显示，绝大多数的程序在加强的设置下，混淆的程度获得了加强。先说下concatstrings这个的NA是混淆前后的similar是1，所以是没有混淆上。有几个程序，例如XXX反而出现了混淆效果的下降，我们认为出现这种情况的原因是BCF对于基本块混淆被指定为概率。而在一个函数中的基本块，并不是混淆概率高的，混淆的次数就一定多。而我们的恢复方法，在三种混淆强度下都取得了接近的效果。恢复CFG和未混淆的CFG之间的差距是由XXX造成的（说个case）

% % 程序在这种方法的混淆下产生了明显的差异性，

% \textbf{\#3. Deobf. Results of CFF:}

% After BCF, We moved our line of sight to the deobfuscation of Control Flow Flatten. While this kind of obfuscating approach being used, the function produces significant differences compare to the unobfuscated one. By default obfuscate setting, the average score of CFG similarity is 0.205562, and some of them are even lower than 0.1. And our deobfuscation result got an average score of 0.806897. After activating basic block split mode, similarity scores are almost all negative correlation, which indicates that the obfuscated CFG is completely different from the unobfuscated one. 

% \begin{figure*}[htbp]
% \centering
% \begin{minipage}[t]{0.15\linewidth}
% \includegraphics[width=\linewidth]{evaluation_pic/16-origin.png}
% \label{fig:side:a}
% \caption{Unobf.}
% \end{minipage}%
% % \begin{minipage}[t]{0.2\linewidth}
% % \includegraphics[width=\linewidth]{pictures/16-1.png}
% % \label{fig:side:b}
% % \end{minipage}
% \begin{minipage}[t]{0.5\linewidth}
% \includegraphics[width=\linewidth]{pictures/16-3.png}
% \label{fig:side:b}
% \caption{Obf.}
% \end{minipage}
% \begin{minipage}[t]{0.25\linewidth}
% \includegraphics[width=\linewidth]{evaluation_pic/16-re.png}
% \caption{Deobf.}
% \label{fig:side:b}
% \end{minipage}
% \end{figure*}


% \textbf{\#4. Example of Deobf. CFF:}

% As the data shows, except a few functions, our system achieves close results on both cases of a same function. We use program 16b-1-1-0-0-dc-2-2-0 as example to illustrate our recover result. This is a function that calculates twice the sum of the ASCII codes corresponding to the string. To clear illustrate, we display the key instructions of each basic block in CFG. 

% The program got a recover result of 0.722222 in both default and enhanced obfuscation. The recovered CFG are shown in figure 12. First, the basic block A in Unobf.'s CFG is a transition block, and we can think that its parent and child node are directly connected. 

% In addition, the two self-loop basic blocks in the original CFG become the loop between the two blocks in the restored result. Like the situation in BCF, key instructions of the two self-loop structures in the unobfuscated function are now implemented in the split-out blocks B and C.


% Now the difference between the result of the recovered and the unobfuscated function lies in edges D and E. But there are almost no operations on edges D and E. In the recovered control flow, due to the splitting of the instructions, the work done by the two branches in the unobfuscated function can be completed by one path. The control flow in recovered CFG can go through the first 3 blocks and 'do nothing'.

% Among programs we analyzed, many unobfuscated functions that originally had a multi-branch structure. But these functions may lose some edges in the recovered CFG. The reason for this phenomenon is that CFF separates constraints and operations during obfuscation, which leads to changes in recovered CFG. So it is also natural to affect the CFG similarity score. In the actual analysis process, such a situation will not affect the analysis, but instead simplify the analysis process.


% % \begin{figure}[htbp]
% % \includegraphics[width=\linewidth]{pictures/sum.png}
% % \label{fig:side:b}
% % \end{figure}

% % \begin{lstlisting}
% % #include <stdio.h>
% % #include <stdlib.h>
% % int main(int argc, char* argv[]) {
% %   int i,j; int sum = 0; const char *str = argv[1];
% %   register const char *s;
% %   for (s = str; *s; ++s) {
% %     sum += *s;}
% %   unsigned int len = (s - str);
% %   for (i = 0; i < len; i++) {
% %     sum += str[i]; }
% %   printf("Sum is: %d\n", sum);
% %   return 0;
% % }
% % \end{lstlisting}
% % 可以看到，除了少数函数，我们的系统在两种情况下取得的结果还是接近的。
% % 而事实上，经过混淆器对控制流的重新分配，这两个分支都可以被合并到他们的父节点对应的另外一条分支上。而原始函数的两个自循环结构的关键指令，在恢复函数的两个循环结构中的拆分出来的块中被实现。
% % 在roman上遇到了一些麻烦，他是个结构非常复杂的函数，当split3的时候有多于400个基本块，对于他的恢复工作不是特别顺利。。。blah


% % 说完了这些，我们对三个mix的情况也进行了分析，这种情况下，我们只关注控制流的恢复情况而不再关注指令替换的对于局部语义的影响。这种情况下三个pass的参数都为默认设置。然后想想怎么说吧
% \textbf{\#5. Deobf. Results of ALL:}

% After completing the separate analysis of the two confusion methods, we implement our deobfuscation approach on the mixture situation of the O-LLVM's three passes. The result is shown in Table too. As data in table shows, 
% % 而恢复出来的cfg score的均值为80%，

% % 这里恢复出来的结果与默认设置的情况基本接近，下面给出二个cases
% % 冒泡排序 + 图 + 分析过程详细解析
% % bkdrhash + 图 + 过程简略解析
% % \begin{figure*}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/gcd-1.png}
% % \label{fig:side:a}
% % \end{minipage}%
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/gcd-3.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/gcd-origin.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/gcd-after.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \caption{gcd}
% % \end{figure*}
% % \begin{figure}
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/cmp_before.png}
% % \label{fig:side:a}
% % \end{minipage}%
% % \begin{minipage}[t]{0.5\linewidth}
% % \centering
% % \includegraphics[width=0.5\linewidth]{pictures/cmp_after.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \caption{CFG merge Rule \uppercase\expandafter{\romannumeral2}}
% % \end{figure}

% %  and the Android projects dataset respectively
% % In order to illustrate the effectiveness and accuracy of our deobfuscating approach, w

% \paragraph{\textbf{Result on Android Projects}}

% \paragraph{CVE}
% After completing the evaluating work of the first two dataset, we put the deobfuscation into the application of the obfuscator in reality. In the researching process, we found that CVE2014 uses the O-LLVM obfuscation method. So we applied our deobfuscating evaluation on dataset C.三个pass都用上后恢复结果


% \section{Case Study}
% \subsubsection{Three Pass Mixed Situation}
% In this section, we are going to discuss the 'all-obfuscated' situation separately. We activated all three passes on 5 program chosen from dataset A.
% % \begin{figure*}[h]\centering
% % \includegraphics[width=.25\textwidth]{pictures/muttable-3-after.png}
% % \includegraphics[width=.25\textwidth]{pictures/muttable-3.png}
% % \includegraphics[width=.25\textwidth]{pictures/muttable-3-before.png}
% % \end{figure*}

% % \begin{figure*}
% % \begin{minipage}[t]{0.3\linewidth}
% % \centering
% % \includegraphics[width=0.3\linewidth]{pictures/muttable-3-before.png}
% % \label{fig:side:a}
% % \end{minipage}%
% % \begin{minipage}[t]{0.3\linewidth}
% % \centering
% % \includegraphics[width=0.3\linewidth]{pictures/muttable-3.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \begin{minipage}[t]{0.3\linewidth}
% % \centering
% % \includegraphics[width=0.3\linewidth]{pictures/muttable-3-after.png}
% % \label{fig:side:b}
% % \end{minipage}
% % \caption{gcd}
% % \end{figure*}

% % 由于时间的限制，我们没有在所有的上面做验证
% % 恢复顺序，先恢复IS，然后找出不透明谓词的块，之后找出所有relevant块，在其中筛去跟不透明谓词块一致的基本块，以避免他们对真实控制流造成的影响，之后进行符号执行，来恢复CF

% \subsubsection{CVE}

==> Automated Deobfuscation of Android Native Binary Code/Section8-Discussion.tex <==
\section{Threats to Validity and Discussion}
\label{sec:discussion}
%  But there are also an important requirement to the input of our system. It needs to ensure that the input binary does not obfuscated by other approach that blurs its semantics, e.g., packing. The defenses of packing in a packed shared library have to be overcome before our system being applied.\haoyu{suggest cut this paragraph}

% \subsubsection{Errors in the underlying framework}
% 由于我们的反混淆工作是以函数为单位的，所以函数基本块的识别非常重要。我们的函数识别是基于ida的识别结果的。由于各个disassembler识别的cfg不一样，可能会对恢复结果造成影响。另外由于我们的符号执行引擎是Angr，对于angr无法识别的或者识别存在误差的指令，也可能会造成结果的不准确。


Although the experimental results suggest that \Name achieves good performance in recovering O-LLVM obfuscated functions, our study, however, carries a few threats to validity.

\textbf{Inherent Limitations of IDA Pro and Angr.}
Since parts of our system build upon several state-of-the-art tools, which might introduce inherent limitations. 
As we perform function-level deobfuscation in this work, it is important to recognize the initial address and the basic blocks in each function. However, it is possible that IDA Pro cannot identify the address of a function accurately, which may lead to inaccuracy of our evaluation. In addition, we rely on Angr to perform symbolic execution, while the instructions that cannot be accurately recognized by Angr will likely cause inaccuracies.
These are the limitations inherited from IDA Pro and Angr, although they rarely occur during our experiments.
%%For example, most of the inconsistencies in our semantic equivalence evaluation were introduced by the incorrect identification of instructions.

\textbf{Semantic Equivalence.}
%%In the previous shown results, not all functions in the \texttt{SE} column have a 100\% \texttt{I/O} matching percentage. We will explain this phenomenon in this section. 
Our experiment suggested that, for a small number of cases, there exist inconsistencies in evaluating the semantic equivalence of deobfuscated binaries and the original ones. We further manually explored these cases and pinpoint the following two reasons.

First, as we use symbolic execution to run the function at the IR level, the \texttt{BL} and \texttt{BLX} instructions sometimes may affect the proper execution of the symbolic execution engine. As shown in Fig.~\ref{fig:uninit}, the semantics of function \texttt{sub\_5F24} is split from the original function. At the very beginning, we try to enter the callee but unfortunately, the execution engine crashed there for quite a few times. Thus, when evaluating semantic equivalence, instead of entering the callee function, we skip them due to the uncertainty of the callee's space. 
Based on the manual analysis of such samples, we observe that the semantics of them are completely recovered by \Name. 
It is worth mentioning that we also skip callee functions in the deobfuscation process, but it will not affect the recovered control flow, as the flow is routed by \(V_{routing}\), which will not be modified cross function or through a callee function.


%%. Because control flow relies on \(V_{routing}\). It will not be modified the cross function or through callee function.

%%We also summarized the samples with such problems and did manual analysis on them. We believe that although there are some differences in \texttt{I/O}, the basic semantics of them are still completely recovered by \Name. Please notice that we also skip callee functions in the deobfuscation process, but it will not affect the recovered control flow. Because control flow relies on \(V_{routing}\). It will not be modified the cross function or through callee function.

% dispatcher中对于寄存器的修改
Second, we saved the symbolic state after each time of symbolic execution in Algorithm 1. Actually, the chopped process of symbolic execution of a block may produce multiple different states before a successor. In the evaluation, \Name only saves one single state, and the state will be updated in the following analysis if it is found to be a non-blank state. It makes our evaluation to be quite effective. However, in some exceptional cases, very few paths may not be found due to the loss of necessary states. 
In our work, we make the number of saved states of one single block configurable, i.e., users could increase the number of states to save.
Increasing the number of saved states will improve our analysis results, as the saved variables are all inherited from the pre-executions.
%%We set the number of saved states of one single block optional for users if they think the increased analyzing time is acceptable. 
%%We believe that increasing the number of saved states will only improve our analysis results because the saved variables are all inherited from the pre-executions.

Although our semantic evaluation approach does not report 100\% identical for several cases, our manually efforts confirmed that all such cases were introduced by the aforementioned reasons, and the recovered programs keep the same semantics actually. 

%%Last, the symbolic execution engine Angr we used may not support some specific opcodes. These opcodes may only appeared in the O-LLVM obfuscated functions, which lead to some exceptions. In this scenario, we set the two outputs of obfuscated and original function are not identical. This situation may affect the \texttt{I/O} percentage to some extent.

%%\noindent \textbf{Extending to other platforms.}
%%Because O-LLVM works in the middle-end of LLVM, it can be applied to many different platforms, as the obfuscation techniques used are the same. It is possible that our system can also be extended to other platforms, such as program analysis on the iOS system. Of course, we may still need to take into consideration the platform-specific optimizations.

% In the shown results of \texttt{I/O} percentage (e.g. values in each "SE" column), we found that not every deobfuscation result is 
% 在前面所展示的结果中，我们可以看到IO一栏中并不是所有样本的io百分比都是100%，这一小节我们将对这一现象进行说明。
% 首先，在验证过程中，由于函数内部调用函数（BL）的存在，使得符号执行的分析变得困难，正如我们之前

% Since our deobfuscating work is applied to each function, 
% the recognition of basic blocks in a function become significantly important. 
% Our function recognition is based on IDA Pro 7.0. 
% But many different disassemblers recognize different CFGs (e.g.,the identification of the end of a function maybe different), it may have a bad impact on the result. 

% Due to the limitation of time, we focus our efforts on deobfuscation of CFF-involved obfuscation. As a result, the implementation of DiANa is only temporarily carried out to the deobfusation of loop equal to 1 (default) in InsSub and BCF. But the principles of deobfuscation which mentioned before are universal.

% \subsubsection{结构复杂的基本块的上下文不好保存}

==> Automated Deobfuscation of Android Native Binary Code/Section9-Conclusion.tex <==
\section{Conclusion}

We have presented a novel approach for deobfuscating Android native code. It uses taint analysis to make semantic-level deobfuscation, and leverages an enhanced flow-sensitive symbolic execution to rebuild the seriously obfuscated control flow. We have implemented our approach in a system called \Name, and demonstrated that \Name could successfully reverse obfuscations performed by O-LLVM with high accuracy. To the best of our knowledge, this is the first work that tackles the problem of Android native code deobfuscation. We believe that our system could become an useful tool for security analysts and researchers to conduct studies including malware detection and program analysis.
